Learning Resource Allocation Policies from Observational Data with an Application to Homeless Services Delivery

We study the problem of learning, from observational data, fair and interpretable policies that effectively match heterogeneous individuals to scarce resources of different types. We model this problem as a multi-class multi-server queuing system where both individuals and resources arrive stochastically over time. Each individual, upon arrival, is assigned to a queue where they wait to be matched to a resource. The resources are assigned in a first come first served (FCFS) fashion according to an eligibility structure that encodes the resource types that serve each queue. We propose a methodology based on techniques in modern causal inference to construct the individual queues as well as learn the matching outcomes and provide a mixed-integer optimization (MIO) formulation to optimize the eligibility structure. The MIO problem maximizes policy outcome subject to wait time and fairness constraints. It is very flexible, allowing for additional linear domain constraints. We conduct extensive analyses using synthetic and real-world data. In particular, we evaluate our framework using data from the U.S. Homeless Management Information System (HMIS). We obtain wait times as low as an FCFS policy while improving the rate of exit from homelessness for underserved or vulnerable groups (7% higher for the Black individuals and 15% higher for those below 17 years old) and overall.

==> background.tex <==

\section{Background}\label{sec:background}
\notepv{I recommend not using bold font for vectors as it is not common in CI I think}\notear{In my previous papers I have used bold font for vectors. We also have an MIO for which I want to use bold for vectors. With bold vectors, things are perhaps more consistent? } 
\notear{I am also not sure where you want the background section to be. I think this paper is different from Nathan Jo's paper as in the intro there are already a lot of material about current system and its issues, model, etc. I can not find a good way to fit this section.}

\noindent\textbf{Treatment Effect Estimation.} Supervised learning is concerned with predicting outcomes for the given features. Within machine learning literature tree-based methods such as CART~\cite{Breiman2017ClassificationTrees} differ from most methods as they produce a partition of the feature space, whereby all samples withing the same partition receive the same prediction. Similarly, causal trees~\cite{Wager2018EstimationForests} partition the feature space into sub-populations that differ in the magnitude of their treatment effects. The method is based on regression trees, modified to estimate the goodness-of-fit of treatment effects. Causal trees~\cite{Wang2017AAnalysis} has been previously used to identify heterogeneous outcome differences between health care providers \cite{Wang2017AAnalysis} across different groups of patients. We also leverage the causal trees to group individuals with similar treatment effect, under each specific resource, into distinct queues. In addition, we use the heterogeneous treatment effect estimations to construct the matching reward for policy optimization. 

\noindent\textbf{Off-policy Evaluation.} Off-policy evaluation is concerned with evaluating a policy $\pi(r \mid \bm X) = \mathbb{P}(r \mid \bm X)$ using data generated by another (potentially unknown) policy. Precisely, we assume to have a set of $N$ i.i.d samples $\mathcal D = \left\{(\bm X_i, R_i, Y_i)\right\}^{N}_{i=1}$ at our disposal, where $\bm X_i \in \mathcal X \subseteq \mathbb R^{d}$ is the feature vector, $R_i \in \mathcal R$ is the received resource and $Y_i \in \mathcal Y \subseteq \mathbb R$ is the observed outcome. We aim to evaluate the policy value $V(\pi) = \mathbb{E}[\sum_{r \in \mathcal R}\pi(r \mid \bm X) Y(\bm X)]$, in which $Y(r) \in \mathcal Y \subseteq \mathbb{R}$ denotes the potential outcome under resource $r$~\cite{Rubin2005CausalOutcomes}. The key challenge in policy evaluation is that we have incomplete knowledge of the outcomes under different resources or interventions. Hence, we are not able to simulate a new policy on the given dataset. The literature on off-policy evaluation offers several estimators to tackle this problem. We first make several assumptions. 
\begin{assumption}[Conditional Exchangeability]
Potential outcomes $\bm Y$ are independent of $R$ given $X$, i.e., $\bm Y \perp R \mid \bm X$. 
\label{assum:exchange}
\end{assumption}
\begin{assumption}[Coverage]
$
\mathbb{P}\left( \mathbb{P}(R = r \mid \bm X = \bm x) > 0 \right) = 1 \; \forall \bm x \in \text{\rm{Supp}}(\bm X).
$
\label{assum:coverage}
\end{assumption}
These assumptions are standard in causal inference which allow the valid inference based on data. Assumption~\ref{assum:exchange} states that, given $\bm X$, the treatment assignment is random, hence, there is no dependence between $R$ and $\bm Y$ suggesting that we measured the right attributes to separate the effect of the outcome from the effect of intervention. Assumption~\ref{assum:coverage} states that the data generating distribution has a strictly positive probability of assigning any treatment to any individual. In Section~\ref{sec:solution}, we discuss the validity of these assumptions in the context of housing allocation data collection. 





\noindent\textit{Direct Method (DM). }
Under Assumption~\ref{assum:exchange}, one can show that 
\begin{equation*}
    \EX[Y(r) \mid \bm X = \bm x] = \EX[Y(r) \mid \bm X = \bm x, R = r] = \EX[Y \mid \bm X = \bm x, R = r].
\end{equation*}
This mean that in order to estimate the expected conditional potential outcome associated with any intervention $r$, we can regress $Y(r)$ on $\bm X$ and $R = r$ which motivates the Direct Method estimator. This estimator forms an estimate $\hat{y}(\bm x, r)$ (e.g., via regression). The policy value is then estimated by 
\begin{equation*}
    \hat{V}^{\text{DM}}(\pi; \mathcal D) = \frac{1}{N}\sum^{N}_{i=1}\sum_{r\in \mathcal R} \pi(r \mid \bm X_i)\hat{y}\left(\bm X_i, r\right). 
\end{equation*}
If $\hat{y}$ is a good approximation of the true expected outcome, then DM is an unbiased estimator of $V(\pi)$. The issue is that $\hat{y}$ is formed without the knowledge of $\pi$ and as a result may perform better in areas that are irrelevant for $V(\pi)$~\cite{Beygelzimer2009TheLabels}.   

\noindent\textit{Inverse Propensity Weighting (IPW). }
The second approach is called \emph{inverse propensity weighting}. Instead of approximating the reward, IPW forms an approximation of the data generating policy, which we denote by $\hat{p}(R = r \mid \bm X = \bm x)$, and uses this estimate to correct for the shift in treatment proportions between the policy that generated the data and the new policy. We recall that $\pi_0$ which is the data generating policy in our problem is deterministic, however, as evident from the data, the policy has not been strictly followed which allows us to estimate $\hat{p}(R = r \mid \bm X = \bm x)$ directly from the data.
\begin{equation*}
    \hat{V}^{\text{IPW}}(\pi; \mathcal D) = \frac{1}{N}\sum^{N}_{i = 1}\frac{\pi(R_i \mid \bm X_i)}{\pi_0(R_i \mid \bm X_{i})}R_{i}, 
\end{equation*}
where $\pi_0(r \mid \bm x)$ the data-generating policy (status-quo policy in the housing setting). It is proven that IPW estimator is an unbiased estimator of the policy value when $\pi_{0}$ is exact. However, it suffers from high variance, and in many applications $\pi_{0}$ should be estimated from data. Additionally, if propensity scores are
arbitrarily close to 0 or 1, IPW converges at rates slower than the parametric models~\cite{Khan2010IrregularEstimation}. 

\noindent\textit{Doubly Robust (DR).}
Proposed by~\cite{Dudik2011DoublyLearning}, \emph{doubly robust} estimator overcomes problems with the previous two estimators.  It has an important property that if at least one of the two estimators, i.e., DM or IPW, is unbiased then the DR estimator is also unbiased. Hence, it increases the chances of reliable inference. 
\begin{equation*}
\hat{V}^{\text{DR}}(\pi; \mathcal D) = \frac{1}{N}\sum^{N}_{i = 1}\sum_{r \in \mathcal R} \pi(r \mid \bm X) \hat{y}(\bm X_i, r) + \frac{1}{N}\sum^{N}_{i = 1} \left(y_i - \hat{y}(\bm X_i, R_i)\right)\frac{\pi(R_i \mid \bm X_i)}{\pi_0(R_i \mid \bm X_{i})}R_{i}. 
\end{equation*}


==> experiments.tex <==
\section{Computational Results}\label{sec:experiments}
We conduct two sets of experiments to study the performance of our approach to design resource allocation policies: \emph{(i)} synthetic experiments where the treatment and potential outcomes are generated according to a known model; \emph{(ii)} experiments on the housing allocation system based on HMIS data for youth experiencing homelessness. We use the causal tree implementation in the \texttt{grf} package in R. We control the partition granularity by changing the \emph{minimum node size} parameter which is minimum number of observations in each tree leaf. We evaluate policies using three estimators from the causal inference literature~\cite{Dudik2011DoublyLearning}:  Inverse Propensity Weighting (IPW) which corrects the mismatch 
between the historical policy and new policy by re-weighting the data points with their propensity values, Direct Method (DM) which uses regression models to estimate the unobserved outcomes, and DR. In addition, we include objective value of Problem~\eqref{prob:MILP} obtained by matching flow and CATE estimates (CT). When models of outcome and propensity are correctly specified, the above estimators are all unbiased~\cite{Dudik2011DoublyLearning}.  
\begin{figure}[t]
    \begin{subfigure}[b]{0.4\textwidth}
    \centering
         \includegraphics[width=\textwidth]{images/value_minProp.pdf}
         \caption{Policy value vs. the minimum propensity weight.}
         \label{fig:small-prop}
    \end{subfigure}\qquad
    \begin{subfigure}[b]{0.4\textwidth}
    \centering
         \includegraphics[width=\textwidth]{images/value_leafSize.pdf}
         \caption{Policy value vs. the number of queues.}
         \label{fig:heter}
    \end{subfigure}  
    \caption{Synthetic data.
Each line corresponds to a different estimator. }
\vspace*{-\baselineskip}
\end{figure}
\subsection{Synthetic Experiments}
We generate synthetic potential outcomes and resource assignments in the HMIS data collected between 2015 and 2017 from 16 communities across the United States~\cite{Chan2017EvidenceYouth}. We use the following setting using vulnerability score $S$ (unless mentioned otherwise):
$\bar{\pi}(\text{SO} |S > 0.2) = 0.3$, $\bar{\pi}(\text{SO} |0.0 < S \leq 0.2) = 0.3$ and $\bar{\pi}(\text{SO} |S \leq 0.0) = 0.3$. Additionally, $\bar{\pi}(\text{RRH} |S > 0.2) = 0.2$, $\bar{\pi}(\text{RRH} |0.0 < S \leq 0.2) = 0.4$ and $\bar{\pi}(\text{RRH} |S \leq 0.0) = 0.3$ and finally, $\bar{\pi}(\text{PSH} |S > 0.2) = 0.5$, $\bar{\pi}(\text{PSH} |0.0 < S \leq 0.2) = 0.3$ and $\bar{\pi}(\text{PSH} |S \leq 0.0) = 0.4$. The potential outcomes are sampled from binomial distributions with probabilities that depend on $S$. For PSH, we use $\mathbb E[Y(\text{PSH}) |S \leq 0.3] = 0.6$, $\mathbb E[Y(\text{PSH}) |0.3 < S \leq 0.5] = 0.2$ and $\mathbb E[Y(\text{PSH}) |0.5 < S] = 0.6$. For RRH, $\mathbb E[Y(\text{RRH}) |S \leq 0.2] = 0.2$, $\mathbb E[Y(\text{RRH}) |0.2 < S \leq 0.7] = 0.6$ and $\mathbb E[Y(\text{RRH}) |0.7 < S] = 0.2$. Finally, $\mathbb E[Y(\text{SO})]= 0$. We evaluate policies obtained by solving  Problem~\eqref{prob:MILP}. We use decision trees for outcome and propensity score models.

%$\bm Y = \text{Binomial}\left(\sigma(\bm \alpha x + \bm \beta)\right)$, where $\bm \alpha = (-20, -10, -5)$ and $\bm \beta = (-1, 1, 2.5)$. 
%creates a natural order between the treatments, i.e., $Y_2 > Y_1 > Y_0$ with high probability. We also simulate a setting where some individuals strictly prefer treatment 1 over treatment 2. We do so by setting $\bm \alpha = (-20, 10, -5)$. 
%Naturally, decision tree (CART) and is a suitable model to fit the propensities and the potential outcomes. The causal tree is also trained with minimum node size $= 40$ (other parameters are set to their default values). 

One of the goals of the synthetic experiments is to compare different estimators in a setting where we observe the potential outcomes. Specifically, we study the performance of the estimators for policy evaluation when propensity values are varied. 
We generate different datasets by changing the  propensity values $\bar{\pi}(\text{PSH}|0.0 < S \leq 0.2) = \alpha$ and $\bar{\pi}(\text{RRH}|0.0 < S \leq 0.2) = 0.7 - \alpha$ for $\alpha \in \{0.02, 0.05, 0.1, 0.2, 0.3\}$ and obtain the optimal policy for each dataset. Figure~\ref{fig:small-prop} shows optimal policy values according to different estimators. We observe that across the $x-$axis range, DR, DM and CT result in similar estimates which also agrees with the ground truth (GT). However, when the minimum propensity score is small ($< 0.05$), IPW diverges from GT. This is consistent with other findings in the literature suggesting that when propensities are too close to 0 or 1, non-parametric estimators tend to have higher variance and converge at a slower rate (with the number of data points)~\cite{Khan2010IrregularEstimation}. 



Next, we investigate the effect of treatment heterogeneity on the value of the optimal policy. In particular, we study how much the granularity of partitions, or the number of queues, impacts the policy value. Figure~\ref{fig:heter} summarizes the results. 
%\notepv{how to read a figure should not be expalined in the text but in the figure caption; this way the figure is independent from the text; only the results from the figure should be described in the text}
When the number of queues is equal to 1, the optimal policy is at its minimum value. In this case, the policy corresponds to an FCFS policy as individuals queue in a single line and are prioritized according to the their arrival times. The optimal policy value gradually increases ($\sim25\%$ according to GT) as the number of queues increases until it flattens. This suggests that by increasing the number of queues, we can leverage the treatment effect heterogeneity across the queues to allocate resources more efficiently.
%This is motivated by the fact that in observational data, a decision-maker has no control over how the treatments are assigned which will impact the inference power. 
%For example, small propensity values ($\mathbb P(\R = \r |\vX = \vx), \forall \r \in \sR$) 
%Next, we empirically study the impact of historical policy propensity values, i.e., $\mathbb P(\R = \r |\vX = \vx), \forall \r \in \sR$, on the performance of the estimators. 
%In observational data, a decision-maker has no control over how the treatments are assigned and some groups may have very low chances of receiving certain treatments which can impact the variance of different estimators, even though they are all unbiased estimators of treatment effect. In fact, existing work shows if propensity values are arbitrarily close to 0 or 1, IPW converges at rates slower than the parametric models~\cite{Khan2010IrregularEstimation}. 

%Earlier, we discussed the conditions that guarantee each of the estimators to be unbiased which involve the accuracy of the learned models. This is typically achieved by selecting a model that has the out-of-sample accuracy. 


%\noindent\textbf{Fairness. }In this section, we study when fairness across queues can lead to improvement in the fairness by protected features.    

\subsection{HMIS Data of Youth Experiencing Homelessness}
We now showcase the performance of our approach to design policies that allocate resource among the U.S. homeless youth. We defer the details on data preparation to the Appendix.

\subsection{Data Pre-Processing and Estimation}
\noindent\textit{Outcome Definition. }We focus on the likelihood of stable exit from homelessness. 
%\begin{figure}
%    \centering
%    \includegraphics[width = 0.4\textwidth]{images/sucess-definition.pdf}
%    \caption{Success definition: We consider the first time an individual leaves the system. Upon leaving the system, an individual can have different destinations namely, Family, Self-resolved, RRH, PSH, Deceased or incarcerated.   Exiting due to incarceration or being deceased are undesirable outcomes, hence we code them as 0. If the individual exits to family, RRH, PSH or self-resolves this is considered as a desirable outcome. However, since some of these exists may be short only those who are housed after a certain amount of time are considered as positive outcome (coded as 1). Finally, there are cases where the exits recorded in the data is due to a move in the system from one service to another which we capture through the last layer. In other words, if there is a record of two consecutive RRH enrollments in the data that are less than 30 days apart, we consider this a move from one to another and counts as 1, however, if the time passed between the interventions is longer than a month, we consider this as 0 outcome.}
%    \label{fig:success-definition}
%\end{figure}
\begin{figure}[t]
    \begin{subfigure}[b]{0.5\textwidth}
    \centering
         \includegraphics[width=0.65\textwidth]{images/sucess-definition.pdf}
         \caption{Success definition flow chart.}
         \label{fig:success-definition}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.5\textwidth}
    \centering
         \includegraphics[width=\textwidth]{images/ceffect_finalscore.pdf}
         \caption{Heterogeneous treatment effect using DR method.}
         \label{fig:ceffect_score}
    \end{subfigure}   
    \caption{HMIS data.}
    \vspace*{-\baselineskip}
\end{figure}
An exit from the system can be to any of the following destinations: ``family,'' ``self-resolved,'' ``RRH,'' ``PSH,'' ``deceased,'' or ``incarcerated.'' Exiting due to incarceration or being deceased are undesirable outcomes and are encoded as $Y = 0$ (left branch). ``Family,'' ``self-resolve,'' ``RRH,'' and ``PSH'' are desirable outcomes but may be temporary exits, meaning that the individual may return to homelessness shortly after. In addition, there are recorded exits that are simply due to a ``move'' in the system from one service to another. 
We distinguish between these cases by checking whether an individual is ``still housed'', i.e., is at the stable exit destination. If re-housed, we consider a 30-day threshold to decide whether it is a return to homelessness ($Y = 0$) or a move in the system ($Y = 1$). This procedure for defining outcome is summarized in Figure~\ref{fig:success-definition}.
%which we capture through the last branching in the tree by checking whether the individual has been rehoused within a month. We check whether an individual is still housed (right branch). 
%In other words, if there is a record of two consecutive RRH enrollments in the data that are less than 30 days apart, we consider this a move from one to another (coded as positive outcome as the individual is still utilizing the resource), however, if the time passed between the interventions is longer than a month, we consider this as 0 outcome. 

\noindent\textit{Propensity Estimation. }
In order to obtain an unbiased estimation of the policy value, IPW and DR approaches rely on propensity values. In our setting, the propensities are unknown but can be estimated from data. This poses a challenge to find a model that fits the data while being well-calibrated. 
We use different statistical models for multi-class classification
%, namely, decision tree, random forest, multinomial logistic regression and neural networks 
to estimate $\mathbb{P}(R = r |\bm X = \bm x), \forall \r \in \sR$. We evaluate models based on the predictive power, calibration, and fairness. For fairness, we adopt the test fairness criteria in~\cite{Chouldechova2017FairInstruments} since evaluating the policy value across different protected groups requires propensity values that are well-calibrated for those groups. We defer the details on model selection to the Appendix. 
We note that the original dataset does not satisfy the positivity assumption. That is, some groups of individuals have only received a subset of the resources. Therefore, for data points with propensities less than 0.001, we follow the status-quo policy and we exclude them from the policy optimization. 

\noindent\textit{Outcome Estimation. }
DM and DR methods rely on a model of the outcome under different resources. We compare an array of models in terms of accuracy, calibration, and test-fairness. The results are summarized in the Appendix.

%We also fit two sets of models, using only the NST vulnerability score and all the covariates available in the data. Including all the features did not result in a significant improvement in the model accuracy except for calibration where including the demographic features helped. However, we only need the calibrated model in the policy evaluation. For the policy optimization and in order to create the queues using the causal tree, we only use the NST score as justified by Proposition~\ref{prop:feature-summarization}. 

\noindent\textit{Heterogenous Treatment Effect Estimation. }
We use causal trees with {minimum node size} {equal to} 15 to estimate the average treatment effects across the NST score range for RRH and PSH. According to Figure~\ref{fig:ceffect_score}, PSH consistently has a higher treatment effect than RRH indicating that it is a more effective resource. Further, the treatment effect of both resources increase with score which suggests that higher-scored individuals benefit more from these resources. We also provide results on the (unbiased) probability of exiting homelessness versus NST score in the Appendix. 

\noindent\textit{Arrival Rate. }
Once the queues are constructed, we estimate the arrival rate of individuals from data. Given the heavy-traffic condition, we calculate the required rate of SO as $\mu_{\text{SO}} = \max\left(\lambda_\sQ - \mu_{\text{RRH}} - \mu_{\text{PSH}}, 0\right)$. \newar{Further, in the HMIS data the resource arrival rates vary with time. In particular, between 2016 and 2017 there is a sharp decrease in the rate of PSH and RRH. Since the rate of resources is often known a-priori to the organisations, in the test data we re-evaluate the arrival rates and re-optimize according to those parameters.}

\subsection{Policy Optimization Results}

We now present the policy optimization results along three distinct objectives: policy value measured in terms of rate of stable exit from homelessness, fairness by race and age, and wait time. Table~\ref{tab:res-total} summarizes the results, where OPT is the optimal policy value without fairness constraints and OPT-fair (race), and OPT-fair (age) represent our method with fairness constraints over race and age, respectively. As baselines, we simulate both a fully FCFS policy and the status quo policy SQ (see Figure~\ref{fig:HMIS-matching}). We also compare with the deployed policy in the data SQ (data). As IPW suffers in small-propensity settings, we exclude it from the estimators.

%We use reliability diagrams to show how well-calibrated different propensity models are. They show the observed frequency of treatments against the predicted probability, providing a quick visual comparison between different models. Specifically, the predicted probabilities are divided up into a fixed number of buckets along the x axis. The number of treatments (class=1) are then counted for each bin (e.g. the relative observed frequency). Finally, the counts are normalized. The results are then plotted as a line plot.
% \begin{table}[htb!]
%     \centering
%     \begin{tabular}{|c|c|c|c|c|}
%     \hline
%     & \multicolumn{4}{c}{Model} \\
%     \cmidrule{2-5}
%     & Multinomial Logistic Regression & Neural Net & CART & Random Forest \\
%     \hline
%     Test Accuracy & 89.9 & 91.1 & 89.9 & 95.2 \\
%     \hline
%     \end{tabular}
%     \caption{Propensity estimation: prediction accuracy on the test set (train/test split using a date cutoff)}
%     \label{tab:propensity}
% \end{table}

%Expected calibration error, maximum calibrations error. 

%\cite{calibration-multiclass}

%\input{realExperimentsNewest}
%\input{realExperimentsNew}
%\input{semiSyntheticExperiments}
%\input{realExperiments}
%\input{realExperimentsScoreandProtected}

% \begin{table}[h]
%     \centering
% \begin{tabular}{P{1.5cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}P{1cm}P{2.1cm}}
% \toprule
% \multicolumn{10}{c}{Training} \\
% \hline
% \multirow{2}{*}{Policy} & \multicolumn{4}{c}{Worse-case Rate of Exiting Homelessness} & \multicolumn{4}{c}{Overall Rate of Exiting Homelessness} & \multirow{2}{*}{Wait Time (Days)} \\
% \cmidrule{2-9}
% & CT & DM & IPW & DR & CT & DM & IPW & DR & \\
% \hline
% OPT &  &  &  &  &  &  &  &  &   \\
% OPT-Fair &  &  &  &  &  &  &  &  &  \\
% FCFS &  &  &  &  &  &  &  &  &  \\
% HUD &  &  &  &  &  &  &  &  &  \\
% HUD (data) &  &  &  &  &  &  &  &  & \\
% \hline
% \multicolumn{10}{c}{Testing} \\
% \hline
% \multirow{2}{*}{Policy} & \multicolumn{4}{c}{Overall Rate of Exiting Homelessness} & \multicolumn{4}{c}{Worse-case Rate of Exiting Homelessness} & \multirow{2}{*}{Wait Time (Days)} \\
% \cmidrule{2-9}
% & CT & IPW & DM & DR & CT & IPW & DM & DR & \\
% \hline
% OPT & 0.76 & 0.71 & 0.75 & 0.72 & 0.70 & 0.71 & 0.74 & 0.70 & \\
% OPT-Fair & 0.76 & 0.71 & 0.75 & 0.73 & 0.75 & 0.72 & 0.75 & 0.72 & \\
% FCFS &  &  &  &  &  &  &  &  &  \\
% HUD &  &  &  &  &  &  &  &  &  \\
% HUD (data) &  &  &  &  &  &  &  &  & \\
% \bottomrule
% \end{tabular}
% \end{table}
% \begin{table}[h]
%     \centering
% \begin{tabular}{P{1.5cm}P{1.5cm}P{1.5cm}P{1.5cm}P{1.5cm}P{1.5cm}P{1.5cm}P{1.5cm}}
% \toprule
% \multirow{2}{*}{Policy} & \multicolumn{3}{c}{Overall Rate of Exiting Homelessness} & \multicolumn{3}{c}{Worse-case Rate of Exiting Homelessness} & \multirow{2}{*}{\makecell{Wait Time \\ (Days)} } \\
% \cmidrule{2-3}\cmidrule{4-7}
% & CT & DM & DR & CT & DM & DR & \\
% \hline
% OPT & \textbf{0.75} & \textbf{0.76} & \textbf{0.75} & 0.69 & \textbf{0.75} & 0.72 & 169.2\\
% OPT-Fair & 0.75 & 0.75 & 0.74 & \textbf{0.74} & \textbf{0.75} & \textbf{0.73} & 169.2\\
% FCFS & 0.66 & 0.64 & 0.66 & 0.59 & 0.61 & 0.64 & 169.0 \\
% HUD & 0.66 & 0.70 & 0.70 & 0.58 & 0.67 & 0.66 & 182.3 \\
% HUD (data) & 0.74 & 0.74 & 0.74 & 0.69 & 0.69 & 0.69 & 200.3\\
% \bottomrule
% \end{tabular}
% \caption{Summary of the policy evaluation results.}
% \label{tab:res-race}
% \end{table}
\begin{table}[t!]
    \centering
\begin{tabular}{P{2.0cm}P{1.5cm}P{1.5cm}P{1.5cm}P{3cm}}
\toprule
\multirow{2}{*}{Policy} & \multicolumn{3}{c}{Rates of Stable Exit from Homelessness} & \multirow{2}{*}{Wait Time (days)} \\
\cmidrule{2-4} & CT & DM & DR & \\
\hline
OPT & 0.76 & 0.74 & 0.75 & 142.67 \\
OPT-Fair (race) & 0.76 & 0.75 & 0.76 & 142.64 \\
OPT-Fair (age) & {0.76} & {0.75} & {0.75} & 142.64 \\
FCFS & 0.68 & 0.68 & 0.66 & 142.64 \\
SQ & 0.66 & 0.63 & 0.63 & 182.21 \\
SQ (data) & 0.73 & 0.73 & 0.73 & 156.77 \\
\bottomrule
\end{tabular}
\caption{{Out-of-sample estimated policy performance} {measured} in terms of rates of stable exit from homelessness and wait times.}
%\notepv{in the table i recommend putting the rates in percent, ie multiplying the numebrs by 100 and writting (\%) in the column name}}
\label{tab:res-total}
\vspace*{-\baselineskip}
\end{table}
From Table~\ref{tab:res-total}, OPT, OPT-fair {(race), and OPT-far (age)} all outperform the baseline policies. Specifically, OPT significantly improves the rate of stable exit from homelessness by 19\% and 13\% (under DR estimates) over SQ and FCFS policies, respectively. Perhaps surprisingly, SQ performs worse than FCFS which is due to how the cut scores are designed. According to SQ individuals with scores 4-7 are matched to RRH. However, the RRH treatment effect is highest for scores above 7 (See Figure~\ref{fig:ceffect_score}). Compared to SQ (data), our policy values are competitive. We improve the wait time over SQ and SQ (data) by 21\% and 9\%, respectively and obtain values similar to FCFS policy. \newar{This is because we have imposed constraints that ensure a single CRP component and subsequently minimum wait time}. As a result, further algorithmic improvement is not possible unless problem inputs, such as resource arrival rates, change. \newar{We note that it is possible to relax the wait time constraints such that the average wait time is not minimum~\cite{Afeche2021OnSystem}. In our setting, this did not lead to an improvement in the policy value.} 
%The optimal objective value of both OPT and OPT-fair is the same (suggesting no price of fairness) and the difference is to sample variance. We also study the wait time. We expect FCFS to have the minimum wait time. Interestingly, our method also achieved similar wait time which suggests that FCFS policy is not Pareto-optimal and we can indeed optimal higher-values policies with minimum wait time. Also, this result shows that it is not possible to improve the wait time unless more the rate of arrival of resources is increased. 
% \begin{table}[h]
%     \centering
% \begin{tabular}{P{2.0cm}P{1.5cm}P{1.5cm}P{1.5cm}}
% \toprule
% \multirow{2}{*}{Policy} & \multicolumn{3}{c}{Worse-case Rate of Exiting Homelessness} \\
% \cmidrule{2-4} & CT & DM & DR \\
% \hline
% OPT & \textbf{0.73} & \textbf{0.73} & 0.72 \\
% OPT-Fair & \textbf{0.73} & \textbf{0.73} & \textbf{0.73} \\
% FCFS & 0.64 & 0.65 & 0.64 \\
% HUD & 0.64 & 0.69 & 0.63 \\
% HUD (data) & 0.62 & 0.62 & 0.62 \\
% \bottomrule
% \end{tabular}
% \caption{Summary of the policy evaluation results when fairness is evaluated across age categories below and above 17 years old.}
% \label{tab:res-age}
% \end{table}
\begin{figure}[t!]
    \begin{subfigure}[t!]{0.47\textwidth}
    \centering
         \includegraphics[width=\textwidth]{images/fairness_race_policy.pdf}
        %\label{fig:outcome-fair-race}
    \end{subfigure}\qquad
    \begin{subfigure}[t!]{0.47\textwidth}
    \centering
         \includegraphics[width=\textwidth]{images/fairness_age_policy.pdf}
             %\label{fig:outcome-fair-age}
    \end{subfigure}  
    \caption{Out-of-sample rates of exit from homelessness {by} race (left panel) and age (right panel) using the DR estimator.}
    \label{fig:outcome-fair}
    \vspace*{-\baselineskip}
\end{figure}
\begin{wrapfigure}{r}{0.3\textwidth}
\centering
    \includegraphics[width=0.25\textwidth]{images/matching-system-new.pdf}
    \caption{Optimal Topology}
    \label{fig:opt-topo}
\end{wrapfigure}
\newar{Finally, we observe that OPT and OPT-fair have similar policy values, indicating a small cost for fairness. This can be explained by the fact that OPT-fair optimizes over queues split by both the protected attribute and risk score, which provides more flexibility to target the resources to different protected groups despite the problem being more constrained.}
Figure~\ref{fig:outcome-fair} compares the worst-case rate of exiting homelessness across age (below and over 17 years old) and racial groups (White, Black, and Other) according to DR estimator and in the test data. First, we observe that an FCFS policy does not necessarily result in 
policies that are fair in terms of their outcomes neither by age nor by race. 
This is because FCFS policies ignore treatment effect heterogeneity. 
In other words, according to {the} FCFS discipline, everyone has the same probability of receiving any {one} of the resource types (fairness in allocation). However, not everyone benefits equally from the resources. Indeed, Black individuals seem to suffer the most under a fully FCFS policy. SQ also yields a low worst-case performance mainly due its low overall performance. SQ (data) has relatively {better} worst-case performance. However, there is still a significant gap between the performance of Black/Other groups and Whites. By explicitly imposing fairness constraints on policy outcomes across protected groups, OPT-Fair significantly improves the performance for the Black and Other groups. Figure~\ref{fig:outcome-fair}, similar observations can be made for fairness by age, where compared to baselines, OPT-Fair exhibits significant improvements in the policy value for those with age below 17.

\begin{wrapfigure}{r}{0.37\textwidth}    \includegraphics[width =0.37\textwidth]{images/matching-system-race.pdf}
    \caption{Optimal and fair matching topology by race.
    Individuals are divided into four different score groups: $S < 6$, $S = \{6\}$, $S = \{7,8\}$, $S > 8$. Queues are constructed based on score groups and race jointly.
    Solid lines indicate that a resource is connected to the entire score group (a collection of queues). Dotted lines indicate connection to a single queue within the score group. For example, SO is only connected to the individuals with $S = \{6\}$ and race White.}
    \label{fig:opt-race}
\end{wrapfigure}

% \begin{figure}[b!]
%     \begin{subfigure}[b]{0.3\textwidth}
%     \centering
%          \raisebox{14mm}{\includegraphics[width=\textwidth]{images/matching-system-race-SO.pdf}}
%          \label{fig:opt-race-SO}
%     \end{subfigure}\hfill
%     \begin{subfigure}[b]{0.3\textwidth}
%     \centering
%          \includegraphics[width=\textwidth]{images/matching-system-race-RRH.pdf}
%          \label{fig:opt-race-RRH}
%     \end{subfigure}\hfill  
%     \begin{subfigure}[b]{0.3\textwidth}
%     \centering
%          \includegraphics[width=\textwidth]{images/matching-system-race-PSH.pdf}
%          \label{fig:opt-race-PSH}
%     \end{subfigure} 
%     \caption{Matching topology split by resource type: left (SO), middle (RRH) and right (PSH). 
%     Individuals are divided into four different score groups: $S < 6$, $S = \{6,7\}$, $S = \{8,9\}$, $S > 9$. Queues are constructed based on score groups and race jointly.
%     Solid lines indicate that a resource is connected to the entire score group (a collection of queues). Dotted lines indicate connection to a single queue within the score group. For example, in the left figure, SO is only connected to the individuals with $S = \{6, 7\}$ and race White.}
%     \label{fig:opt-race}
% \end{figure}


%This is consistent with existing studies on adverse outcomes for Black people experiencing homelessness. 
% \begin{wrapfigure}{r}{0.3\textwidth}
%     \centering
%     \includegraphics[width=0.25\textwidth]{images/matching-system-new.pdf}
%     \caption{Optimal Topology}
%     \label{fig:opt-topo}
% \end{wrapfigure}
% \begin{wrapfigure}{r}{0.25\textwidth}
%     \centering
%     \includegraphics[width = 0.25\textwidth]{images/matching-system_age-new.pdf}
%     \caption{The optimal fair topology with respect to age when we require the topology to not depend on the age group of the individuals.}
%     \label{fig:opt-age-noDependece}
% \end{wrapfigure}
% \begin{figure}[b!]
%     \begin{subfigure}[b]{0.25\textwidth}
%     \centering
%         \includegraphics[width=\textwidth]{images/matching-system-new.pdf}
%         \caption{Optimal topology}
%         \label{fig:opt-topo}
%     \end{subfigure}\qquad
%     \begin{subfigure}[b]{0.27\textwidth}
%     \centering
%          \includegraphics[width=\textwidth]{images/matching-system_age-new.pdf}
%          \caption{Optimal, fair topology (age)}
%          \label{fig:opt-age-noDependece}
%     \end{subfigure}\qquad  
%     \begin{subfigure}[b]{0.27\textwidth}
%     \centering
%          \includegraphics[width=\textwidth]{images/matching-system_age-new.pdf}
%         \caption{Optimal, fair topology (race)}
%         \label{fig:opt-race-noDependence}
%     \end{subfigure} 
%     \caption{Matching topologies for optimal policy with and without fairness constraints. }
%     \label{fig:topology}
% \end{figure}


% \newar{In ~\cite{kleinberg2016inherent, chouldechova2017fair} it has been shown that imperfect predictors cannot simultaneously satisfy equal odds and
% calibration unless the groups have identical base rates, i.e. rates of positive outcomes.}
% \begin{figure}[t!]
%     \begin{subfigure}[b]{0.5\textwidth}
%     \centering
%          \includegraphics[width=0.75\textwidth]{images/matching-system.pdf}
%          \caption{Optimal topology}
%          \label{fig:opt-topo}
%     \end{subfigure}\hfill
%     \begin{subfigure}[b]{0.5\textwidth}
%     \centering
%          \includegraphics[width=0.75\textwidth]{images/matching-system_age.pdf}
%          \caption{Optimal topology with fairness constraints on age}
%          \label{fig:age-topo}
%     \end{subfigure}   
% \end{figure}
%\noindent\textbf{Learning using DM Method}
%\notepv{it would be more intuitive to have the more vulnerable individuals and the more supportinve interventions at the top}

We now present a schematic diagram of OPT and OPT-fair matching topologies. Figure~\ref{fig:opt-topo} is the matching topology corresponding to OPT policy. Compared to SQ, OPT uses different cut points on NST score, specifically for the lower-scoring individuals. Across the four score groups, we observe a gradual transition from eligibility for a more resource-intensive intervention (PSH) to a basic intervention (SO). Figure~\ref{fig:opt-race} depicts OPT-fair topology for fairness on race, in which queues are constructed using the joint values of NST score and race. According to this figure, PSH is matched to all individuals with scores above 9 as well as mid-scoring Black individuals, i.e., $6 \leq \text{score} \leq 9$. RRH is connected to every individual in the mid-score range. Our modeling strategy uses the protected characteristics in order to ensure fairness. This is motivated by discussions with our community advisory board, including housing providers/matchers and people with past history of homelessness, who suggested that in order to create a fair housing allocation system there ought to be special accommodations for historically disadvantaged people. 
\begin{wrapfigure}{r}{0.23\textwidth}
    \centering
    \includegraphics[width=0.23\textwidth]{images/matching-system_race.pdf}
    \caption{Fair topology when queues are not divided by race.}
    \label{fig:race-topo}
\end{wrapfigure}
Our policies align with affirmative action policies that take individuals' protected attributes into account in order to overcome present disparities of past practices, policies, or barriers by prioritizing resources for underserved or vulnerable groups. In this regard, recently HUD restored Affirmatively Furthering Fair Housing rule that requires ``HUD to administer its programs and activities relating to housing and urban development in a manner that affirmatively furthers the purposes of the Fair Housing Act'', extending the existing non-discrimination mandates~\cite{2021RestoringCertifications}. 




Our approach can also be extended to non-affirmative policies. This is possible by imposing constraints that ensure a topology has the same connections to all  protected groups within a score group. Such constraints are expressible as linear constraints and can be easily incorporated in Problem~\eqref{prob:MILP}. We demonstrate the result for fairness on race in Figure~\ref{fig:race-topo}. We observe that all individuals who belong to a certain queue, regardless of their race, are eligible for the same types of resources. However, as a result of combining the queues, the worst-case policy value across the racial groups decreases from 0.76 to 0.73 which still outperforms SQ and SQ (data) with worse-case value of 0.61 and 0.69, respectively. We defer the results for fairness by age to Appendix.
%\notepv{since all people in the same queue have the same treatemnt effect, how can you have unfair policies if you don't differentiate queues by race?}
%from 0.74 to 0.69 which still outperforms the SQ (data) (0.64). 
%We imposed such constraints and the results are presented in Figure~\ref{fig:opt-age-noDependece} where resources are directed to queues defined by NST score regardless of the age of the individuals. We note that a result of these constraints, we may loose some of the performance boost in fairness. In the case of Figure~\ref{fig:opt-age-noDependece}, the worst-case performance decreased from 0.74 to 0.69 which still outperforms the SQ (data) (0.64). We present the topology results for fairness by race in the Appendix. 
% \begin{figure}[t!]
%     \begin{subfigure}[t]{0.33\textwidth}
%     \centering
%          \includegraphics[width=\textwidth]{images/matching-system-age-SO-new.pdf}
%          \label{fig:opt-age-SO}
%     \end{subfigure}\hfill
%     \begin{subfigure}[t]{0.33\textwidth}
%     \centering
%          \includegraphics[width=\textwidth]{images/matching-system-age-RRH-new.pdf}
%          \label{fig:opt-age-RRH}
%     \end{subfigure}\hfill  
%     \begin{subfigure}[t]{0.33\textwidth}
%     \centering
%          \includegraphics[width=\textwidth]{images/matching-system-age-PSH-new.pdf}
%          \label{fig:opt-age-PSH}
%     \end{subfigure} 
%     \caption{The matching topology split by resource type: left (SO), middle (RRH) and right (PSH). The solid line indicates that the resource is connected to the entire queue. The dotted line indicates connection to a sub-group within the queue. For example, in the left figure, SO is only connected to the individuals with NST = 6 and age over 17.}
%     \label{fig:opt-age}
% \end{figure}
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width = 0.25\textwidth]{images/matching-system_age-new.pdf}
%     \caption{The optimal fair topology with respect to age when we require the topology to not depend on the age group of the individuals.}
%     \label{fig:opt-age-noDependece}
% \end{figure}

%\notepv{PLEASE ADD ACKNOWLEDGEMENTS FOR THE PAPER YOU WILL POST ONLINE: ask eric about how to thank people in the advisory board. see paper i sent you}

\section{Research Ethics and Social Impact}\label{sec:discussion}
Recently, there has been a significant growth in algorithms that assist decision-making across various domains~\cite{Rice2012DiscriminatoryColor, Goodman2018MachineReasoning, Simonite2020MeetCollege, Monahan2016RiskSentencing}. Homelessness is a pressing societal problem with complex fairness considerations which can benefit greatly from data-driven solutions. As empirical evidence on ethical side effects of algorithmic decision-making is growing, care needs to be taken to minimize the possibility of indirect or unintentional harms of such systems. 
We take steps towards this goal. Specifically, we propose \emph{interpretable} data-driven policies that make it easy for a decision-maker to identify and prevent potential harms. Further, we center our development around issues of \emph{fairness} that can creep into data from different sources such as past discriminatory practices. %Such biases may vary over time and across different populations. 
We provide a flexible framework to design policies that overcome such disparities while ensuring efficient allocations in terms of wait time and policy outcome.


There are also crucial consideration before applying our framework in real-world. Our approach relies on several key assumptions about the data. Specifically, the consistency assumption requires that there is only one version of PSH, RRH, and SO. In practice, different organizations may implement different variants of these interventions. For example, combining substance abuse intervention with PSH and RRH. Such granular information about the interventions, however, is not currently recorded in the data which may impact CATE estimates. Further, the exchangeability assumption requires that there are no unobserved confounders between treatment assignment and outcomes. Even though our dataset consists of a rich set of features for each individual, in practice, unobserved factors may influence the allocation of resources which calls for more rigorous inspection of service assignment processes. Unobserved confounders may lead to biased estimates of treatment effects which in turn impacts the allocation policies.
In addition, our dataset consists of samples from 16 communities across the U.S., which may not be representative of new communities or populations. Hence, the external validity of such policies should be carefully studied before applying to new populations. Finally, there are other domain-specific constraints that we have not considered as they require collecting additional data. For example, resources can not be moved between different CoCs. We leave such considerations to future work.


\begin{acks}
P. Vayanos and E. Rice gratefully acknowledge support from the Hilton C. Foundation, the Homeless Policy Research Institute, and the Home for Good foundation under the ``C.E.S. Triage Tool Research \& Refinement'' grant. P. Vayanos is also grateful for the support of the National Science Foundation under CAREER award number 2046230.
Finally, we thank the project's community advisory board for helpful discussions throughout the development of this work. 
\end{acks}

%certain allocations may not be feasible due to geographic constraints (a resource becomes available in a location different from the allocatee's).
%This is specifically pertinent when we think about biases that can creep into the models. For example, discriminatory practices may change over time and from one community to another. Finally, 


% Choice of problem 
% Data collection
% Data assumption
% Model 
% Results 

%\lipsum


==> introduction.tex <==
% \notepv{i think the paragraph below should come before the previous paragraph: basically explain how things are currently done; what are some good things about it (e.g, it's interpretable; and what are some bad things about it; discuss how the current policy is not actually adopted and why). this will help motivate what you are doing.}
% \notepv{i do not like that suddently in the middle of the intro we switch the focus to homeless youth; is this a paper about homeless youth? if so that should be made clear; Else, please talk about homelessness in general even if you use homeless youth as a running example} \notepv{in addition there should be a paragraph somewhere saying that your approach can be applied to other problems too, outside of homelessness}
% \notepv{you had mentioned interpretability before; does that not matter here? are we less interpretable?}\notear{the baselines are FCFS, status-quo policy and the data. I think interpretability may not be relevant here as the baselines can also be expressed as some form of resource eligibility structure and are interpretable.} 
\section{Introduction}
%\notepv{i recommend starting by more general resource allocation systems and then focus on housing, i.e. to show that our methods here are actually more general}

We study the problem of designing policies to effectively match heterogeneous individuals to scarce resources of different types. We consider the case where both individuals and resources arrive stochastically over time. Upon arrival, each individual is assigned to a queue where they wait to be matched to a resource. This problem arises in several public systems such as those providing social services, posing unique challenges at the intersection of {efficiency and fairness. In particular, the joint characteristics of individuals and their matched resources determine the effectiveness of an allocation policy, making it crucial to match individuals with the right type of resource. Furthermore, when a resource becomes available, a decision-maker should decide whom among the individuals waiting in various queues should receive the resource which impacts the wait time of different individuals. In addition, since there are insufficient resources to meet demand, there are inherent fairness considerations for designing such policies.}

%The individual's intrinsic characteristics and the characteristics of their assigned resource, determine the efficiency of the policy. 

We are particularly motivated by the problem of allocating housing resources among individuals experiencing homelessness. According to the U.S. Department of Housing and Urban Development (HUD), more than 580,000 people experience homelessness on a given night~\cite{Henry2020AHAR:Exchange}. The Voices of Youth Count study found youth homelessness has reached a concerning prevalence level in the United States; one in 30 teens (13 to 17) and one in 10 young adults (18 to 25) experience at least one night of homelessness within a 12-month period, amounting to 4.2 million persons a year~\cite{Morton2018PrevalenceStates}. Housing interventions are widely considered as the key solution to address homelessness~\cite{U.S.Dept.ofHousingandUrbanDevelopment2007TheReport}. In the U.S., the government funds programs that assist homeless using different forms of housing interventions and services~\cite{2015OpeningHomelessness}. The HMIS database collects information on the provision of these services.
%People experiencing homelessness are subject to a wide range of physical and mental health problems which negatively impact their individual well being~\cite{Burt2007Community-wideEvidence}.  
%The Homeless Management Information System (HMIS) database collects information on the provision of these services.


\begin{figure}[t!]
    \centering
    \includegraphics[width = 0.35\textwidth]{images/HMIS-matching-system-1.pdf}
    \caption{NST-recommended resource allocation policy utilized by housing allocation agencies in the homelessness context.
    The policy is in the form of a resource eligibility structure. According to this figure, individuals with score eight and above qualify for PSH, score 4 to 7 are assigned to the RRH wait list and finally individuals who score below 4 are not assigned to any of the housing interventions.}
    \label{fig:HMIS-matching}
    \vspace*{-\baselineskip}
\end{figure}
%Second is resource heterogeneity. Specifically, there are different levels of housing assistance and supportive services namely long-term resource-intensive housing programs or Permanent Supportive Housing (PSH), short-term rental subsidy programs or Rapid-ReHousing (RRH), and minimal services that meet basic needs which we refer to as Service Only (SO). These interventions have varying effectiveness for different individuals, making it crucial to match the individuals with the right type of intervention. Finally, resources are allocated in a dynamic environment where both individuals and resources arrive stochastically over time. A resource allocation policy that ignores this uncertainty may perform poorly in practice. For example, we may allocate a costly intervention (e.g., PSH) to an individual with low vulnerability which could be more effective for a more vulnerable individual entering the waiting list in near future. The above factors together determine the success and impact of a housing allocation policy. In this work, we evaluate a policy along three main dimensions: \emph{interventions effectiveness} measured in terms of the expected number of individuals with safe and stable exit from homelessness, \emph{fairness} defined flexibly as either the rate of allocated resources or \newar{the expected outcome} across different social groups (e.g., race, age, etc.), and the \newar{expected} \emph{wait time}. 

% third paragraph
Unfortunately, the number of homeless individuals in the U.S. far exceeds the available resources which necessitates strategic allocation to maximize the intervention's effectiveness. Many communities have attempted to address this problem by creating coordinated community responses, typically referred to as Coordinated Entry Systems (CES). In such systems, most agencies within a community pool their housing resources in a centralized system called a Continuum of Care (CoC). A CoC is a regional or local planning body that coordinates housing and services funding—primarily from HUD—for people experiencing homelessness.
%Risk assessment tools are widely adopted for this purpose which measure \newar{an} individual's vulnerability based on their history of housing and homelessness, risks, socialization and daily functions, and wellness~\cite{Hsu2019UnderstandingAnalysis}.
%Due to the scarcity of resources, many communities use risk assessment tools to determine individuals' need for housing assistance and match them with appropriate resources.  
Individuals in a given CoC who seek housing are first assessed for eligibility and vulnerability and those identified as having the greatest need are matched to appropriate housing resources~\cite{Rice2017AssessmentYouth}. For example, in the context of youth homelessness, the most widely adopted tool for assessing vulnerability is the Transition Age Youth-Vulnerability Index-Service Prioritization Decision Assistance Tool (TAY-VI-SPDAT): Next Step Tool (NST), which was developed by OrgCode Consulting, Corporation for Supportive Housing (CSH), Community Solutions, and Eric Rice. OrgCode claims that hundreds of CoC's in the USA, Canada and Australia have adopted this tool~\cite{Orgcode2015TransitionYouth}. After assessment, each individual receives a vulnerability score ranging from 0 to 17. One of the main challenges that CoC's face is how to use the information about individuals to decide what housing assistance programs should be available to a particular homeless individual. In many communities, based on the recommendations provided in the NST tool documentation, individuals who score 8 to 17 are considered as ``high risk'' and are prioritized for resource-intensive housing programs or Permanent Supportive Housing (PSH). Those who score in the 4-7 range are typically assigned to short-term rental subsidy programs or Rapid-ReHousing (RRH) and those with score below 4 are eligible for services that meet basic needs which we refer to as Service Only (SO)~\cite{Rice2018LinkingYouth}. Figure~\ref{fig:HMIS-matching} depicts how the individuals are matched to resources according to the status-quo policy. 


The aforementioned policy can be viewed as a \emph{resource eligibility structure} as from the onset, it determines the resources an individual is eligible for. Such policies have the advantage of being interpretable, i.e., it is easy to explain why a particular allocation is made. Earlier work shows that most communities follow the policy recommendations when assigning housing~\cite{Rice2018LinkingYouth}. However, controversy has surrounded the use of these cut scores and as of December 2020, OrgCode has called for new approaches to using the data collected by HMIS~\cite{OrgCode2020TheVI-SPDAT}. There is also an overwhelming desire on the part of HUD to design systematic and data-driven housing policies, including the design of the cut scores and the queues that they induce~\cite{2015OpeningHomelessness}. Currently, the cut scores are not tied to the treatment effect of interventions or the relative arrival rate of individuals and resources in the respective queues. This is problematic as it is not evidently clear that assigning high-scoring and mid-scoring individuals to particular housing
interventions, such as PSH or RRH, actually increases their chances of becoming stably housed. Additionally, there may not be enough resources to satisfy the needs of all individuals matched to a particular resource, resulting in long wait times. Prolonged homelessness may in turn increase the chances of exposure to violence, substance use, etc., or individuals dropping out of the system. 

In particular, OrgCode and others have called for a new equity focus to how vulnerability tools are linked to housing allocation \cite{OrgCode2020TheVI-SPDAT,Milburn2021InequityHomelessness}. Despite recent efforts to understand and mitigate disparities in homelessness, current system suffers from a significant gap in the prevalence of homelessness across different groups. 
%Studies show that most racial minority groups experience homelessness at higher rates than Whites. For example, Blacks represent 13\% of the general population but account for more than 40\% percent of people experiencing homelessness~\cite{Fusaro2018RacialStates}. 
For example, studies show that most racial minority groups experience homelessness at higher rates than Whites~\cite{Fusaro2018RacialStates}. Also, recent work has revealed that PSH outcomes are worse for Black clients in Los Angeles~\cite{Milburn2021InequityHomelessness} and based on the same HMIS data used in present study, Black, Latinx, and LGBQ youth have been shown to experience worse housing outcomes~\cite{Hill2021AnStatus}. Addressing these disparities requires an understanding of the distribution of the individuals vulnerability to homelessness, the heterogeneity in the treatment affect and the associations with protected attributes such as race, gender, or age. 


%Recent work has shown that PSH outcomes are worse for Black clients in Los Angeles~\cite{Milburn2021InequityHomelessness} and based on the same HMIS data used in present study, Black, Latinx, and LGBQ youth have been shown to experience worse housing outcomes~\cite{Hill2021AnStatus}.

%\notepv{you have not talked about disparities clearly; this just comes up casually at the end of this paragraph but should be one of your central points; in my opinion there should be a dedicated paragraph about it. } 


% fourth paragraph
%In this work, we propose to leverage historical data on the deployed policy and its outcomes to learn fair, interpretable and efficient policies. 

%In doing so, we ensure that our policies are interpretable, in the sense that it is easy to explain why a particular allocation was made. 

%We note that this problem arises in broader settings where we need to allocate scarce heterogeneous resources under fairness and wait time considerations such as U.S. kidney allocation system or the U.S. public housing program. Our proposed framework is applicable to all of these contexts. We now summarize our main contributions:

%We introduce a framework that \notepv{what does this mean?} maintains the key aspects of housing allocation in the context of homelessness, specifically, our model has the following features: i):  resources are allocated dynamically as they arrive ii) \notepv{what does this mean and why do we care?} they abstract away from the problem of minimizing waiting times. 



%, creating a unique opportunity to leverage the data to learn the heterogeneous treatment effect of various housing interventions and design more effective policies. 

%\notepv{also if the focus is going to be on homelessness only, then we should justify the assumptions we make, e.g. conditional exchangeability early on}

In this work, we build on the literature on causal inference and queuing theory and propose a methodology that uses historical data about the waitlisted individuals and their allocated resources to optimize resource allocation policies. 
%that take policy effectiveness, fairness and wait time into account. 
We make the following contributions:
\begin{itemize}
    \item We model the policy optimization problem as a multi-class multi-server queuing system between heterogeneous individuals and resources that arrive over time. We extend the literature on queuing theory by proposing a data-driven methodology to construct the model from observational data. Specifically, we use tools from modern causal inference to learn the treatment effect of the interventions from data and construct the queues by grouping individuals that have similar average treatment effects.  %As a result, upon arrival each individual is assigned to a queue which determines the\newar{ir} eligibility for different types of resources.
    \item We propose interpretable policies that take the form of a {resource eligibility structure}, encoding the resource types that serve each queue.
    We provide an MIO formulation to optimize the eligibility structure that incorporates flexibly defined fairness considerations or other linear domain-specific constraints. The MIO maximizes the policy effectiveness 
    %measured in terms of the expected number of individuals with safe and stable exit from homelessness 
    and guarantees minimum wait time.
    \item Using HMIS data, we conduct a case study to demonstrate the effectiveness of our approach. Our results indicate superior performance along policy effectiveness, fairness and wait time. Precisely, we are able to obtain wait time as low as a fully FCFS policy while improving the rate of exit from homelessness for traditionally underserved or vulnerable groups (7\% for the Black individuals and 15\% higher for youth below 17 years old) and overall. 
\end{itemize}
The remainder of this paper is organized as follows. In Section~\ref{sec:literature}, we review the related literature. %In Section~\ref{sec:background} we provide the necessary background on data-driven optimization using observational data. 
In Section~\ref{sec:statement}, we introduce the policy optimization problem. In Section~\ref{sec:solution}, we propose our data-driven methodology for solving the policy optimization problem. Finally, we summarize our numerical experiments and present a case study using HMIS data on youth experiencing homelessness in Section~\ref{sec:experiments}. Proofs and detailed numerical results are provided in the Appendix.


==> literaturereview.tex <==


% \notepv{is abandoning the queue the same as receiving service?}\notear{the model for abandonment is such that a customer will abandon the queue after a random duration that follows a fixed probabilistic distribution. So I think it is different from the model we are considering. I think it could be another addition to the model but different from the SO queue that we have}
% \notepv{the question here is why we don't need to vonsider abandonment}
% \notear{I am not sure I understand this question. I think abandonment could be important to model. In our data we have individuals with unknown outcomes which could be due to system abandonment. So, I can not make a claim that it does not happen. Modelling abandonment is not the subject of this paper but something to consider in future work. Is this what you mean by this question?}
% \notepv{you cite my paper with Chaitanya; but we have an MCMS system there.. what's the connection? i thought our queuing system model here is actually similar to the one in that paper} \notear{Not sure about this comment. I think in your paper the focus is on wait time estimation and not policy optimization. For this reason I did not include more information.}
\section{Literature Review}\label{sec:literature}

This work is related to several streams of literature which we review. Specifically, we cover queuing theory as the basis of our modelling framework. We also position our methodology within the literature on data-driven policy optimization and causal inference. We conclude by highlighting recent works on fairness in resource allocation. 
%\paragraph{Queuing Theory}
%\notepv{this section should cite Trichakis paper on kidney allocation and my paper with Javad on housing allocation; these are very related to what you do so very important to contrast} \notepv{i now see that you have a separate section on data-drive policy optimization; it may be good to say to the reader in advance what the streams you will review are and what the difference between section 2.1 and 2.3 is. e.g., i am not sure why some works go in 2.3 rather than 2.1 and vice versa.}

A large number of scarce resource allocation problems give rise to one-sided queuing models. In these models, resources are allocated upon arrival, whereas individuals queue before being matched. Examples are organ matching~\cite{Bandi2019RobustSystems} and public housing assignment~\cite{Kaplan1984ManagingHousing,Arnosti2020DesignAllocation}.
%In the public housing setting in particular, households applying for public housing are allowed to specify those housing projects in which they are willing to live. When a public housing unit becomes newly available, of those households willing to live in the associated housing project, the one that has been waiting the longest is offered the unit~\cite{Kaplan1984ManagingHousing, Kaplan1988ARENEGING}. Most studies study the queuing system under pre-specified compatibility structure~\cite{Castro2020MatchingSolution,Zhan2018Many-serverFCFSALIS}. 
One stream of literature studies dynamic matching policies to find asymptotically optimal scheduling policies under conventional heavy traffic conditions~\cite{Mandelbaum2004SchedulingC-rule, Ata2013OnCosts}. Another stream focuses on the system behavior under FCFS service discipline aiming to identify conditions that ensure the stability of the queuing system and characterize the steady-state matching flow rates, i.e., the average rate of individuals of a given queue (or customer class) that are served by a particular resource (server)~\cite{Fazel-Zarandi2018ApproximatingLaw, Castro2020MatchingSolution}. 
These works only focus on minimizing delay and do not explicitly model the heterogeneous service value among the customers.
Recently,~\cite{Ding2021ARewards} studied one-sided queuing system where resources are allocated to the customer with the highest score (or index), which is the sum of the customer’s waiting score and matching score. The authors derive a closed-form index that optimizes the steady-state performance subject to specific fairness considerations. Their proposed fairness metric measures the variance in the likelihood of getting service before abandoning the queue. Contrary to their model, we consider FCFS policies subject to resource eligibility structures which we optimize over. Our model is based on the policies currently being implemented for housing allocation among homeless individuals \newar{that target resources to heterogeneous individuals by explicitly imposing an eligibility structure}. \newar{Our policies are interpretable by design as upon arrival the resources that an individual is eligible for is known, making it easy to explain why a certain allocation has or has not been made}. Further, the proposed model allows for a more general class of fairness requirements commonly used in practice including fairness in \emph{allocation} and \emph{outcome}. \newar{It is noteworthy that our model is different from common allocation models in the public housing setting where targeting of the resources can be considered as implicit, i.e., individuals with different levels of need make different choices about where to apply and what to accept themselves~\cite{Arnosti2020DesignAllocation, Arnosti2019HowHousing}}.

Our approach builds upon~\cite{Afeche2021OnSystem}, in which the authors study the problem of designing a matching topology between customer classes and servers under a FCFS service discipline. They focus on finding matching topologies that minimize the customers' waiting time and maximize matching rewards obtained by pairing customers and servers. The authors 
%study the system under the heavy-traffic condition and 
characterize the average steady-state wait time across all customer classes in terms of the structure of the matching model, under heavy-traffic condition. %To circumvent the computational complexity of computing matching rewards under a FCFS service discipline, 
They propose a quadratic program (QP) to compute the steady-state matching flows between customers and servers and prove the conditions under which the approximation is exact. We build on the theoretical results in~\cite{Afeche2021OnSystem} to design resource eligibility structures that match heterogeneous individuals and resources in the homelessness setting. Contrary to the model  in~\cite{Afeche2021OnSystem}, we do not assume that the queues or the matching rewards are given a priori. Instead, we propose to use observational data from historical policy to learn an appropriate grouping of individuals into distinct queues, estimate the matching rewards, and evaluate the resulting policies.

Another stream of literature focuses on designing data-driven policies, where fairness considerations have also received significant attention due to implicit or explicit biases that models or the data may exhibit~\cite{Bertsimas2013FairnessTransplantation,Dickerson2015FutureMatch:Environments,Rahmattalabi2021FairApproach, Keymanesh2021Fairness-awareDecision-Making}. In~\cite{Bertsimas2013FairnessTransplantation}, the authors propose a data-driven model for learning scoring policies for kidney allocation that matches organs at their time of procurement to
available patients. Their approach satisfies linear fairness constraints approximately and does not provide any guarantees for wait time. In addition, they take as input a model for the matching rewards (i.e., life years from transplant)to optimize the scoring policy.
In~\cite{Azizi2018DesigningResources}, the authors propose a data-driven mixed integer program with linear fairness constraints to solve a similar resource allocation which provides an exact, rather than an approximate, formulation. They also give an approximate solution to achieve faster run-time. We consider a class policies in the form of matching topologies that is different from scoring rules and is more closely related to the policies implemented in practice. Such policies offer more interpretability as individuals know what resources they are eligible for from the onset. Several works have considered interpretable functional forms in policy design. For example, in~\cite{Bertsimas2019OptimalTrees, Jo2021LearningData}, the authors consider decision trees and develop techniques to obtain optimal trees from observational data. Their approach is purely data-driven and do not allow for explicit modelling of the arrival of resources, individuals which impact wait time. In the homelessness setting, our work is closely related to~\cite{Kube2019} which proposes a resource allocation mechanism to match homeless households to resources based on the probability of system re-entry. In this work, the authors provide a static formulation of the problem which requires frequent re-optimization and does not take the waiting time into account. In~\cite{Nguyen2021ScarceJustice}, the authors propose a fairness criterion that prioritizes those who benefit the most from a resource, as opposed to those who are the neediest and study the price of fairness under different fairness definitions. Similar to~\cite{Kube2019}, their formulation is static and does not yield a policy to allocate resources in dynamic environments. 
%Fairness considerations have also received significant attention due to implicit or explicit biases that models or the data may exhibit. Axiomatic and fairness concerns have been considered across several domains such as kidney exchange both in the static~\cite{Dickerson2014PriceExchange} and online setting~\cite{Dickerson2015FutureMatch:Environments}, social-network based interventions~\cite{Rahmattalabi2019ExploringProblems, Rahmattalabi2021FairApproach}, and housing allocation~\cite{Nguyen2021ScarceJustice}. 
%\newar{\cite{keymanesh2021fairness}}
%\newar{envy-freeness in sequential decision-making with heterogeneous resources and utilities\cite{sinclair2021sequential}}.

%\newar{Kathryn to add more to the literature review\cite{keymanesh2021fairness}}

%\notepv{this section does not sound like a literature review; it sounds like a tutorial. Therefore, it does not fit in a section on literature review; Having a tutorial is ok, but then it should be in a ``background'' section. For example, it Nathan Jo paper, we have a background section on this stuff: \url{http://www.optimization-online.org/DB_FILE/2021/08/8569.pdf} but then the literature review is focused on reviewing the literature. I recommend reorganizing. Also, there should be a literature review on causal inference that is different from this tutorial. That literature review should cite e.g., the paper of Nathan Jo on prescriptive trees and similar literature and contrast with these works}


==> problemformulation.tex <==
% \notepv{would be good to have a figure of MCMS system to illustrate the ideas}
% \notepv{need to use parentheses for matrices, not square brackets; also, when defining a new math symbol/function, use ``:='' rather than ``=''; makes it easier for the reader to know what is going on}
% \notear{For the bracket I adopted the notation in Afeche paper. Happy to change it if you still believe it should be parentheses.}
% \notepv{i think these constraints have been proposed by trichakis, if so need to cite him}
% \notepv{is it possible to ensure that there is always at least one matching that satisfies this? you give an example in the next few sentenses but first need to explain} \notear{Not sure what this comment means}
% \notepv{are the two problems equivalent? does the number of CRP come up anywhere?}\notear{not quite equivalent because the flows are approximated. The constraints impose a single CRP.}
%\notear{make parameters dependent on $\P$. Need to re-read the whole thing.}
%\notepv{in some of the examples, you said that we need to have different queues for different protected groups; how do you do that?}
\section{Housing Allocation as a Queuing System}\label{sec:statement}

\subsection{Preliminaries}
We model the resource allocation system as an infinite stream of heterogeneous individuals and resources that arrive over time. Each individual is characterized by a (random) feature vector $\vX \in \sX \subseteq \mathbb R^n$ and receives an intervention $\R$ from a finite set of treatments indexed in the set $\sR$. We note that $\sR$ may include ``no intervention'' or minimal interventions such as SO in the housing allocation setting.
Using the potential outcomes framework~\cite{Rubin2005CausalOutcomes}, each individual has a vector of potential outcomes $Y(r) \in \mathcal Y \subseteq \mathbb R \; \forall \r \in\sR$, where $Y(\r)$ is an individual's outcome when matched to resource $\r$. 

%\notepv{need to explain that it is a mapping from the covariate space to a probability of receiving each resource; or is it a random mapping from the covariate space to a choice of resource? or is it a random mapping from the covariate times resource space to a number?}

We assume having access to $N$ historical observations $\mathcal D := \left\{(\bm X_i, R_i, Y_i)\right\}^{N}_{i=1}$, generated by the deployed policy, where $\vX_i \in \sX$ denotes the feature vector of the $i$th observation, $\R_i \in \sR$ is the resource assigned to it and $Y_i = Y_i(\R_i)$ is the observed outcome, i.e., the outcome under the resource received. {A (stochastic) policy $\pi(\r|\vx): \sX \times \sR \rightarrow [0, 1]$ maps features $\vx$ to the probability of receiving resource $\r$. We define the value of a policy as the expected outcome when the policy is implemented, i.e.,
$V(\pi) := \EX[\sum_{r \in \mathcal R}\pi(r | \bm X)Y(r)]$.}
%where the expectation is over the joint distribution of 
%\notepv{it would be better to introduce this joint distribution $\mathbb P$ earlier and then say this is the expectation with respect to $\mathbb P$}
%$\vX, Y(r) \; r \in \sR$ and $\pi$. 
A major challenge in evaluating and optimizing policies is that we cannot observe the counterfactual outcomes $Y_i(r), r \in \sR, r \neq \R_i$ of resources that were not received by data point $i$. Hence, we need to make further assumptions to identify policy values from historical data. In Section~\ref{sec:solution}, we elaborate on these assumptions and propose our methodology for evaluating and optimizing policies from data.
%\notepv{this paragraph ends really abruptly and you don't tell us if or when you will tell us about these assumptions; I suggest that we resolve this cliffhanger}%Causal inference allows us to formalize these assumptions.

%\notepv{when defining mathematical symbols, i propose to use ``:='' rather than ``=''; it's more precise} 
%\notepv{it is too late to say this now no? this is what the paragraph should start with}\notepv{it is not clear how to chose the number of queues}
We model the system as a multi-class multi-server (MCMS) queuing system where a set of resources $\sR$ serve a finite set of individual queues indexed in the set $\sQ$. Upon arrival, individuals are assigned to different queues based on their feature vector. For example, in the housing allocation setting and according to the recommended policy the assignment is based on the vulnerability score. We use $\P : \sX \rightarrow \sQ$ to denote the function that maps the feature vector to a queue that the individual will join. We refer to $\P$ as the \emph{partitioning function} (as it partitions $\sX$ and assigns each subset to a queue) and note that it is unknown a priori. In this work, we consider partitioning functions in the form of a binary trees similar to classification trees, due to their interpretability~\cite{Azizi2018DesigningResources}. We assume that individuals arrive according to stationary and independent Poisson processes and that inter-arrival time of resources follows an exponential distribution. \newar{These are common assumptions in queuing theory for modeling arrivals, however, they may not fully hold in practice in which case, it is possible to use re-optimization to adapt to the changing environment.}
%\notepv{why is it ok to assume that this holds in the housing example?? there are many assumtpikons that are not justified}
We use $\bm \lambda := (\lambda_1, \dots, \lambda_{|\sQ|})$ and $\bm \mu := (\mu_1, \dots, \mu_{|\sR|})$ to denote the vector of arrival rates of individuals and resources, respectively. We define $\lambda_{\sQ} := \sum_{\q \in \sQ} \lambda_{\q}$ and $\mu_{\sR} := \sum_{\r \in \sR} \mu_{\r}$ as the cumulative arrival rates of individuals and resources, respectively. Without loss of generality, we assume that  $\lambda_\q > 0 \; \forall \q \in \sQ$ and $\mu_\r > 0 \; \forall \r \in \sR$. 


\subsection{Matching Policy}
Once a new resource becomes available, it is allocated according to a resource eligibility structure that determines what queues are served by any particular resource. The resource eligibility structure can be  represented as a matching topology $\vM := [\m_{\q\r}] \in \{0,1\}^{|\sQ| \times |\sR|},$ where $\m_{\q\r} = 1$ indicates that individuals in queue $\q$ is eligible for resource $\r$. Resources are assigned to queues in an FCFS fashion subject to matching topology $\vM$. For a partitioning function $\P$ and matching topology $\vM$, we denote the allocation policy by $\pi_{\P, \vM}(\r | \vx)$. We concern ourselves with the long-term steady state of the system. Proposition~\ref{prop:steady-state} gives the necessary and sufficient conditions to arrive at a steady-state. 

\begin{proposition}[\citet{Adan2014AAbandonments}, Theorem 2.1]
Given the MCMS system defined through $(\mathcal Q, \mathcal R, \bm \lambda, \bm \mu, \vM)$, under the FCFS service discipline matching $\vM$ admits a steady state if and only if the following condition is satisfied:
\begin{equation*}
    \mu_{\mathscr{R}} - \sum_{\r \in \mathscr{R}}\sum_{\q \in \sQ_{\mathscr{R}}(\vM)} \lambda_{\q} > 0 \quad \forall \mathscr{R} \subseteq \sR.
\end{equation*}
The left-hand side is the cumulative arrival rate of resources in $\mathscr{R}$ in excess of the cumulative arrival rate of all the queues in $\sQ_{\mathscr{R}}$, where $\sQ_{\mathscr{R}}$ is the set of queues that are only eligible for resources in $\mathscr{\R}$, i.e., $\sQ_{\mathscr{R}} = \{\q \in \sQ : \sum_{\r \in \sR\setminus\mathscr{R}}\m_{\q\r} = 0\}$.
\label{prop:steady-state}
\end{proposition}
We define the set of \emph{admissible matching topologies} as those that satisfy the inequality in Proposition~\ref{prop:steady-state}. 
In the housing allocation problem, we assume that SO resources are abundant, i.e., $\mu_{\sR} - \lambda_{\sQ} > 0 $. \newar{In other settings, it is possible to create an auxiliary resource queue corresponding to no intervention.} The abundance assumption ensures that there exists at least one admissible matching: the fully connected matching topology $\m_{\q\r} = 1\; \forall \q \in \sQ, \r \in \sR$ and is necessary in order to avoid overloaded queues. %\newar{Without it, the system does not arrive at the steady-state, resulting in growing wait times and policies that do not perform as expected in the test data.}
In practice housing resources are strictly preferred. As a result, we propose to study the system under the so-called \emph{heavy traffic} regime, where the system is loaded very close to its capacity and we assume that the system utilization parameter $\rho := \mu_{\sR}/\lambda_{\sQ}$ approaches 1, i.e., $\rho \rightarrow 1$. In general, we assume that $\bm \lambda$ and $\bm \mu$ are such that $\lambda_{\sQ} = \rho \mu_{\sR}$. This assumption will additionally make the analytical study of the matching system more tractable. In particular, in~\cite{Afeche2021OnSystem}, the authors propose a quadratic program to approximate the exact steady-state flows of the stochastic FCFS matching system
under heavy traffic conditions. They enforce the steady-state flows in an optimization model to find the optimal matching topology using KKT optimality conditions. We adopt the same set of constraints in Section~\ref{sec:optimization} where we present the optimization formulation. 
We let $\vF := [\f_{\q\r}] \in \mathbb{R}_{+}^{|\sQ| \times |\sR|}$ denote the steady-state flow, where $\m_{\q\r} = 0 \Rightarrow \f_{\q\r} = 0$. Given a partitioning function $\P$, the policy associated with a matching topology $\vM$ is equal to $\pi_{\P, \vM}(\r | \bm x) = \f_{\q\r}/\sum_{\r\in\sR}{\f_{\q\r}} = \f_{\q\r}/\lambda_{\q}$, in which $\q = \P(\vx)$ and the second inequality follows from the flow balance constraints.
%indicating that individuals who belong to the same queue have the same probability of receiving different resources. 
In Proposition~\ref{prop:policy_value} we show how the policy value can be written using the matching model parameters and treatment effect of different interventions. We define the conditional average treatment effect (CATE) of resource $\r$ and queue $\q$ as $\tau_{\q\r} := \mathbb{E}[Y(\r) - Y(1) | P(\vX) = \q] \; \forall \r \in \sR, \q \in \sQ$, in which $\r = 1$ is the baseline intervention. {In many applications, the baseline intervention corresponds to ``no-intervention'' (also referred to as the control group)}. In the housing allocation context, we set $\r=1$ to be the SO intervention.
%as it is a non-housing intervention.

%We note that since all the incoming flow to a queue $\q$ is served by the resources we have $\lambda_{\q} = \sum_{\r \in \sR}\f_{\q\r}$. \newar{something is off here}
%Given $\P$ and $\vM$, we can estimate the FCFS flow rates using the quadratic program in~\cite{Afeche2021OnSystem}.
\begin{proposition}
Given a partitioning function $\P$, an MCMS model $(\sQ, \sR, \bm \lambda, \bm \mu, \vM)$, and the steady-state FCFS flow $\vF$ under FCFS discipline, the value of the induced policy $\pi_{\P,\vM}$ is equal to: 
\begin{equation*}
    V(\pi_{\P, \vM}) = \frac{1}{\lambda_{\sQ}}\sum_{\q \in \sQ} \sum_{\r \in \sR} \f_{\q\r}\tau_{\q\r} + C,
\end{equation*}
where 
%$\tau_{\q\r} = \mathbb{E}[Y(\r) - Y(1) |P(\vX) = \q], \forall \r \in \sR, \q \in \sQ$ is the conditional average treatment effect (CATE) of resource $\r$ and queue $\q$ and 
$C$ is a constant that depends on the expected outcome under the baseline intervention.
\label{prop:policy_value}
\end{proposition}

%Using the KKT optimality conditions for the quadratic program, one can formulate the problem of finding optimal topologies under the two distinct objectives, i.e.,  policy value and wait time as an MIO~\cite{Afeche2021OnSystem}.

\subsection{Policy Optimization}

%\notepv{i think you also assume the arrival rates are known; I do not think you will relax the assumption that P is known; you will just propose a way to construct P}\notear{If P and the joint distribution is known the arrival rates will be known as well.}

We now introduce the policy optimization problem under the assumption that the joint distribution of $\bm X, Y(\r), \r \in \sR$ as well as the partitioning function $\P$ is known. In Section~\ref{sec:solution}, {we propose a methodology to construct $\P$. Furthermore, we describe how we can use historical data to optimize new policies.}
%We first consider a simplified case with no fairness or wait time considerations. 
%In order to formulate the problem, we further assume that the partitioning function $\P$ is given. 
\begin{equation}
    \sP(\P) := \max_{\vM \in \sM} V(\pi_{\P, \vM}).
    \label{prob:policy-optimization}
\end{equation}
In the above formulation, $\sM$ is the set of feasible matching topologies. In addition to the constraints that impose steady-state flow, we incorporate fairness and wait time constraints in the set $\sM$ which we describe next. 
%We use $\sF$ and $\sW$ to denote the set of fairness and wait time constraints. 
%and policy value $V(\pi_{P, \vM})$ is the objective function. 
%In order to further impose fairness and wait time requirements, we propose to augment Problem~\ref{prob:policy-optimization} with additional constraints which we explain next.

%In Proposition~\ref{prop:policy_value}, both $C$ and denominator $\lambda_{\mathcal Q}$ are constants and can be removed from Problem~\ref{prob:policy-optimization}. 

%The goal is to design a policy $\pi(r |\bm x) = \mathbb{P}(R = r |\bm X = \bm x)$

% Consider a multiclass, multiserver (MCMS) queuing system between a set of distinct resources and 

% where a set of $R$ distinct servers, indexed by j
% 1, . . . , M, serve K customer classes, similarly indexed
% by i  1, . . . , K. Associated with the ith customer class,
% there is an infinitely sized queue that is populated by
% all customers of that class, which we shall refer to as
% i-customers. Customers of each class can only be served
% by a fixed subset of servers. Let (i) ⊂ {1, . . . , M} be the
% (nonempty) set of servers eligible to serve i-customers.
% Correspondingly, let (j) ⊂ {1, . . . , K} be the set of
% queues or customer classes for which the jth server is
% eligible. 





%We assume to have access to a set of $N$ historical observations $\mathcal D = \left\{(\bm X_i, R_i, Y_i)\right\}^{N}_{i=1}$, generated by the deployed policy, where $\bm X_i \in \mathcal X \subseteq \mathbb R^{d}$ denotes the feature vector of the $i$th observation, $R_i \in \mathcal R$ is the resource assigned to it and $Y_i = Y_i(R_i)$ is the observed outcome, i.e., the outcome under the received resource. The goal is to design a new policy $\pi: \mathcal X \rightarrow \mathcal R$ using dataset $\mathcal D$. Since we have no control over the historical resource allocations, the outcomes $Y_i(r), r \neq R_i$ remain unobserved. 




%We assume that we have access to historical observations $\mathcal D = \left\{(\bm X_i, R_i, Y_i)\right\}^{N}_{i=1}$ generated by the deployed policy, where $Y_i = Y_i(R_{i})$ is the observed outcome given resource $R_i$ \notepv{need to clarify the challenge here; need more details}. 

\iffalse
\begin{table}[t!]
    \centering
    \begin{tabular}{ lcc }
    \toprule
    Description & Notation & Definition
    \\
    \hline
    Set of queues & $\mathcal Q$ & $\{1, \dots, Q \}$ 
    \\
    Set of resources & $\mathcal R$ & $\{1, \dots, R\}$ 
    \\
    Arrival rates of individuals across queues & $\bm \lambda$ & $\{\lambda_1, \dots, \lambda_Q\}$ 
    \\
    Arrival rate of resources & $\bm \mu$ & $\{\mu_1, \dots, \mu_R\}$
    %Matching reward between individual queue $q$ and resource queue $r$ & $\bar{Y}$ & $\left[\bar{Y}_{qr}\right] \in \mathbb{R}^{Q \times R}$ 
    \\
    Feasible matching & $\bm M$ & $\left[m_{qr}\right] \in \{0,1\}^{Q \times R}$ 
    \\
    Flow rate  & $\bm F(\bm M)$ &  $\left[f_{qr}(\bm M)\right] \in \mathbb{R}_{+}^{Q \times R}$
    \\
    Set of queues that can be served by $\mathscr{R} \subseteq \mathcal R$ & $U_{\mathscr{R}}(\bm M)$ &  $\{q \in \mathcal Q |m_{qr} = 1\; \forall r \in \mathscr{R} \}$
    \\
    Cumulative rate of arrival for a subset of resources $\mathscr{R} \subseteq \mathcal{R}$ & $\mu_{\mathscr{R}}$ & $\sum_{r \in \mathscr{R}}\mu_{r}$
    \\
    Cumulative rate of arrival for a subset of queues $\mathscr{Q} \subseteq \mathcal{Q}$ & $\lambda_{\mathscr{Q}}$ & $\sum_{q \in \mathscr{Q}}\lambda_{q}$
    \\
    \bottomrule
    \end{tabular}
    \caption{Notation \notepv{do we really need this table? do we really need to define big Lambda? big mu? big M? why is M and F not bold? what does "individuals queues" mean? is it different than "queues"? why is there an s at the end of individuals? in the penultimate line, why are we summing over t? the ntoation $M_{qr}$ seems inconsistent with $m_{qr}$} \notear{I prefer to keep the table until the we cover the entire paper. All of these notations come up later.}}
    \label{tab:notation}
\end{table}
\fi
%Inspired by the status-quo policy, we consider the setting where upon arrival individuals are assigned to a queue each of which are matched to a subset of resources. For a particular resource, we refer to the set of individual queues that are matched to it as the \emph{eligible queues} for that resource.  \newar{edit here} 
%\notepv{please revise the entire paragraph and in particular the order in which you introduce things and define new terminology carefully; please see section 2 of my MCMS paper for an example} 
%We consider an interpretable class of policies that take the form of a service compatibility structure, i.e., a matching topology \notepv{it does not make sense to talk about matching topology when you have not yet defined the queues and servers; see for example Section 2 in my MCMS paper for example of how to introduce everything}. We are inspired by the status-quo policy in which upon arrival individuals are assigned to a queue based on their NST score. Each queue is eligible for a predetermined subset of resources \notepv{again please see my MCMS paper for an example of how to phrase this}. When a new resource arrives, it will be allocated to the \newar{first} individual \newar{to have} arrived \newar{in any one of the queues it is eligible to serve}. 
%We are inspired by the current status-quo policies, illustrated in Figure~\ref{fig:HMIS-matching}, which categorizes individuals based on their NST scores which in turn determines the resources that an individual is eligible for. Figure~\ref{fig:HMIS-matching} depicts the how the individuals are matched to resources according to the status-quo policy. \notepv{again, please do not focus on the homelessness example and if you have already defined this policy in the introduction, there is no need to redefine it} Individuals with score eight and above qualify for PSH, scores 4 to 7 are assigned to the RRH wait list and finally individuals who score below 4 are assigned to SO. Upon procurement of a new PSH resource, it will be allocated to the individual who has waited the longest among those who score 8 or above. 
%For a policy to be efficient (efficiency will be precisely defined shortly), both the break points and the matchings to different resources should be tied to their respective outcomes.
%We proceed in two steps: we first create the queues, by partitioning the feature space of the individuals \notepv{need to explain why this makes sense! right now it reads as a not very sensible idea}.
%Each individual will be then mapped \notepv{not clear what you mean by mapped; maybe say that we will effectively partition the feature space so that each individual belongs to one subset of this partition which in turn is associated with a queue} to one of the queues. We define $P : \mathcal X \rightarrow \mathcal Q := \{1, \dots, Q\}$ to be the mapping \notepv{need to be more explicit here; maps covariates to a queue that the invididual will join}, where $Q$ is the maximum allowable number of queues (decision-maker may set a bound on the number of queues for operational and interpretability purposes). We refer to $P$ as the \emph{partitioning function}. 
%we use $\mathcal P$ to denote the set of such mappings.
%$\mathcal X = \cup^{Q}_{q = 1}\mathcal X_q$ where $Q$ is the maximum allowable number of queues (some queues may be empty and therefore not utilized). For example a decision-maker may set a bound on the number of queues for operational and interpretability purposes. 
%\notepv{no need to repeat this here; we must have stated something along those lines in the previous paragraph} Next and given the queues, individuals wait until resources become available and are matched to them according the FCFS principle. \notepv{what policy are you talking about? this has not been introduced. Please be thoughtful about the order in which you itnroduce things: would someone that has not talked to you be able to follow what you are writting?} 
%Precisely, the policy $\pi_{M}(r |\bm x)$ is equal to $\mathbb{P}(r |\bm X = \bm x)$, i.e., the probability that individual $\bm x$ receives $r$. We note that $M = M(P)$ \notepv{what is the object on the right? it does not seem to be in your table} \notepv{i do not understand this statement; why is M a fucntion of P?}, however, we drop the dependence on $P$ to minimize notational overhead. 
%The policy is governed by the matching process, i.e., the matching topology and the FCFS resource allocation discipline. We use the tuple $(\mathcal Q,\mathcal R, \bm \lambda,\bm \mu)$ to define the matching model \notepv{i do not like that some things are input (data) and some things can be controled by us and yet we put them together in a tuple -- why is this needed?} \notepv{do we really need all this? also, i am against using tables of notation and for sure using a table summarizing notation is not a reason to not explain the notation in the text} \notepv{this paragraph is really hard to follow} . Table~\ref{tab:notation} provides the description of the parameters. Additionally, we denote a matching between the individual queues and the resource queues by $M$ \notepv{you are using M before and you are defining it here.. please reorder}. Once $P$ is fixed, it is easy to see that the matching model is fully specified \notepv{I do not see this; i thought P tells you which queue each individual goes to and then M tells you which queues are matched to each server} . 
%As mentioned in the introduction, in the housing allocation policy optimization problem we proceed in two steps. First, we wish to find a partitioning function $P$ to construct the matching model. Next, we aim to find an optimal policy $\pi_{M}$ (that depends on the matching topology $M$). Given $M$, we can estimate the FCFS flow rates using the quadratic program in~\cite{Afeche2021OnSystem}. The policy is then equivalent to $\pi_{M}(r |\bm X) = f_{qr}/\lambda_{q}$, where $q = P(\bm X)$. We note that since all the incoming flow to the individual queues $q$ is served by the resources we have $\lambda_q = \sum_{r \in \mathcal R}f_{qr}$. Finally, it holds if $m_{qr} = 0 \Rightarrow f_{qr} = 0$.   
% We now introduce the population version of the policy optimization problem that assumes the joint distribution of $(\bm X, \bm Y)$ is known and given. Later in Section~\ref{sec:solution}, we relax this assumption. We also discuss how we propose to learn the partitioning function $P$.  
% \begin{equation}
%     \mathcal{H}(P) := \max_{M \in \mathcal M(P)} V(\pi_{M}; P).
%     \label{prob:policy-optimization}
% \end{equation}
% In the above formulation, $M$ is the matching topology, $V(\pi_{M})$ is the efficiency of the policy $\pi_{M}$ and $\mathcal M$ is a set of admissible policies which further includes constraints to impose fairness and wait time constraints. When clear from the context, we drop the dependence on $P$. We now define the objective value and the constraints precisely. 
%\section*{Solution Approach}\label{sec:solution}
%\noindent\textbf{Efficiency. }We define the expected rate of people exiting homelessness as $V(\pi_M) = \EX[\sum_{r \in \mathcal R}\pi_{M}(r |\bm X)Y(r)]$. In Proposition~\ref{prop:policy_value} we show how the policy value can be written using the matching model parameters.
% We define the matching rewards $\bar{Y}_{qr} = \mathbb{E}[Y(r) ]$ as the average probability of safe exit from homelessness if an individual from from queue $q$ is matched with a resource of type $r$ (possible if $M_{qr} = 1$). 
%
\paragraph{Fairness}
In this work, we focus on group-based notions of fairness which have been widely studied in recent years in various data-driven decision making settings~\cite{Rahmattalabi2019ExploringProblems,Azizi2018DesigningResources,Nguyen2021ScarceJustice,Bertsimas2013FairnessTransplantation}. Formally, we let $G$ be a random variable describing the group that an individual belongs to, taking values in $\sG$. For example, $\G$ can correspond to protected features such as race, gender or age. It is also possible to define fairness with respect to other features, such as vulnerability score in the housing allocation setting. We give several examples to which our framework applies.
%\newar{Parity-based notions of fairness strive for equal outcome across different groups. Finally, we can impose fairness in the \emph{allocation} of resources or in the \emph{system outcome}, i.e., policy value. Next, we describe several fairness constraints that can be incorporated in Problem~\eqref{prob:policy-optimization}. We start by fairness in outcome as the more general case.}
\begin{example}[Maximin Fairness in Allocation]
Motivated by Rawls theory of social justice~\cite{Rawls1999TheoryEdition}, maximin fairness aims to help the worst-off group as much as possible. Formally, the fairness constraints can be written as
\begin{equation*}
    \sum_{\q \in \sQ_\g} \f_{\q\r} \geq w \quad \forall \g \in \sG, \r \in \sR,
\end{equation*}
where $w$ is the minimum acceptable flow across groups and $\sQ_\g \subseteq \mathcal Q$ is a subset of queues whose individuals belong to $\G = \g$. If queues contain individuals with different values of $g$, one should separate them by creating multiple queues with unique $g$. 
By increasing the parameter $w$, one is imposing more strict fairness requirements. This parameter can be used to control the trade-off between fairness and policy value. It can also be set to the highest value for which the constraint is feasible. 
%According to the above inequalities, for every resource the cumulative flow to each group should be at least $w$.
\end{example}

\begin{example}[Group-based Parity in Allocation]
Parity-based fairness notions strive for equal outcomes across groups. 
\begin{equation*}
    \left|\sum_{\q \in \sQ_\g} \f_{\q\r} - \sum_{\q \in \sQ_{\g'}} \f_{\q\r}\right| \leq \epsilon \quad \forall \g, \g' \in \sG, \r \in \sR.
\end{equation*}
In words, for every resource the difference between the cumulative flow between any pair of groups should be at most $\epsilon$,
%, where $\epsilon$ is the tolerance on deviation from parity across groups. 
where $\epsilon$ can be used to control the trade-off between fairness and policy value.
\end{example}

\begin{example}[Maximin Fairness in Outcome]
For every group, the policy value should be at least $w$.
% \begin{equation*}
%     %\EX\left[\sum_{\r \in \sR}\pi_{\P, \vM}(r |\bm X)Y(r) \,\middle\vert\, \G = \g \right] \geq w \; \forall \g \in \sG,  
%     \EX\left[\sum_{\r \in \sR}\pi_{\P, \vM}(r |\vX)Y(r) \,\middle\vert\, \G = \g \right] \geq w \quad \forall \g \in \sG, 
% \label{def:fairness-maximin-outcome}
% \end{equation*}
\begin{equation*}
 \frac{1}{\lambda_{\mathcal Q_g}}\sum_{\q \in \mathcal Q_g} \sum_{\r \in \sR} \f_{\q\r}\tau_{\q\r} \geq w \quad \forall \g \in \sG.
\end{equation*}
% \begin{equation*}
%     \EX\left[\sum_{\r \in \sR}\pi_{\P, \vM}(\r |\bm X)Y(\r) \,\middle\vert\, \G = \g\right] = \frac{1}{\lambda_{\mathcal Q_g}}\sum_{\q \in \mathcal Q_g} \sum_{\r \in \sR} \f_{\q\r}\tau_{\q\r} + C \quad \forall \g \in \sG, 
% \end{equation*}
%\notepv{kind of repetitive}According to the above definition, we aim to improve the matching outcome for the worst-off group(s) by requiring performance $w$ for every group. 
%Using the result in Proposition~\ref{prop:policy_value}, we can rewrite the left-hand-side expression in terms of the matching parameters. 
%where the left-hand side is the policy value for group $g$. 
\end{example}

\begin{example}[Group-based Parity in Outcome]
The difference between the policy value for any pair of groups is at most $\epsilon$.
\begin{equation*}
    %\left|\EX\left[\sum_{r \in \sR}\pi_{\P, \vM}(\r |\bm X)Y(\r) \,\middle\vert\, \G = \g\right] -  \EX\left[\sum_{r \in \sR}\pi_{\P, \vM}(\r |\vX)Y(\r) \,\middle\vert\, \G = \g'\right]\right| \leq \epsilon \quad \forall \g, \g' \in \sG.
     \left|\frac{1}{\lambda_{\sQ_\g}}\sum_{\q \in \sQ_\g} \sum_{\r \in \sR} \f_{\q\r}\tau_{\q\r} - \frac{1}{\lambda_{\sQ_{\g'}}}\sum_{\q \in \sQ_\g'} \sum_{\r \in \sR} \f_{\q\r}\tau_{\q\r} \right|  \leq \epsilon \quad \forall \g, \g' \in \sG.
\label{def:fairness-parity}
\end{equation*}
\end{example}
In the experiments, we focus on fairness in outcome due to treatment effect heterogeneity. In other words, it is important to match individuals with the right type of resource, rather than ensuring all groups have the same chance of receiving any particular resource. Further, we adopt maximin fairness which guarantees Pareto optimal policies ~\cite{Rahmattalabi2021FairApproach}.
%It has been previously shown that parity-based fairness in decision-making problems may result in policies that are not Pareto optimal~\cite{Hu2020FairWelfare,Rahmattalabi2021FairApproach} leading to wastage of resources. We adopt maximin fairness which does not suffer from this limitation~\cite{Rahmattalabi2021FairApproach}. 
% \begin{theorem}
% Suppose $Y(r) \perp \bm X |P(\bm X) = q, \forall r \in \mathcal{R}, q \in \mathcal{Q}$. It holds that:
% \begin{align*}
%     & \EX\left[\sum_{r \in \mathcal R}\pi_M(r |\bm X)Y(r) \,\middle\vert\, P(\bm X) = q\right] - \EX\left[\sum_{r \in \mathcal R}\pi_M(r |\bm X)Y(r) \,\middle\vert\,  P(\bm X) = q'\right] = 0, \; \forall q, q' \in \mathcal{Q}
%     \\
%     \Rightarrow & \EX\left[\sum_{r \in \mathcal R}\pi_M(r |\bm X)Y(r) \,\middle\vert\, G = g\right] -  \EX\left[\sum_{r \in \mathcal R}\pi_M(r |\bm X)Y(r) \,\middle\vert\, G = g'\right]  = 0, \; \forall g, g' \in \mathcal{G}.
% \end{align*}
% \end{theorem}
%This theorem informally states that if a policy is fair across the queues, in the sense of Definition~\ref{def:fairness-parity}, the policy subsequently satisfies the fairness constraints by protected groups. 
% \begin{observation}
% Fully FCFS policy satisfies fairness in allocation but not necessarily in the outcome. 
% \label{obs:fcfs-fair}
% \end{observation}
%In order to prove the above observation, consider a simple queuing system with two individual queues (e.g., low-risk and high-risk) and two types of resource (e.g., SO and PSH). For simplicity, we assume the arrival rates are all equal. Let us further assume that individual queues coincide with the sensitive group membership, i.e., individuals in the low-risk (resp. high-risk) queue belongs to $G=1$ (resp. $G=2$). Under a fully FCFS discipline, each queue has equal chance of receiving either type of 
%So far, we have assumed that the partitioning function $P$ and subsequently the queues $Q$ are given. Additionally, we assume all the matching parameters including the $\bar{Y}$. 
%\noindent\textbf{assumptions. } We note that while the status-quo policy policy is a deterministic policy by design (based on the NST score category, there is only one type of resource that the individual is eligible for), the historical data shows deviations from this policy. We leverage the randomness in the intervention assignment which as we show allows us to meet the coverage assumption.
%Our approach is flexible in how the groups are defined, making it suitable for different domains. The groups can be either defined based on the traditionally marginalized groups or e.g., African American or Black individuals, vulnerable groups and their intersections, e.g., Black females, and finally we can require fairness by the NST score and score groups or the queues themselves. 
%nerability score of the youth so that, independently of their backgrounds and past experiences, youth are equally likely to transition into stable housing For example, one could require that the probability of a stable exit for a youth in the system should be equal across different races, or independent of the vul. 
%We also study the system in the steady-state. In Section~\ref{sec:background},  Proposition~\ref{prop:steady-state} we provide the necessary and sufficient conditions for the system to arrive at the steady-state. Henceforth, we drop the dependence on time.
%Similarly, we consider an implementable class of policies that take the form of a service compatibility structure, i.e., the policy induces a partition on the feature space of the individuals $\mathcal X$ to create distinct individual queues (wait lists), each of which will be eligible for a subset of resources. We define $\mathcal P : \mathcal X \rightarrow \mathcal Q$ as a function that assigns the individual $\bm x$ to one of the queues in the set $\mathcal Q$. 
%Following the FCFS discipline, the policy assigns arriving resources to the individuals on the wait lists. Explicitly, we use $\pi(\bm X; M)$ to denote the policy corresponding to matching topology $M$. We note that in our setting $\mathcal P$ is not determined a priori (queues are not given). The only information available is the number of desired queues. We propose to find the function $\mathcal P$ as part of the policy optimization which we describe in more detail in Section~\ref{sec:solution}. 
%We are inspired by the current status-quo policies, illustrated in Figure~\ref{fig:HMIS-matching}, which categorizes individuals based on their NST scores which in turn determines the resources that an individual is eligible for. According to Figure~\ref{fig:HMIS-matching}, individuals with score eight and above qualify for PSH, scores 4 to 7 are assigned to the RRH wait list and finally individuals who score below 4 are assigned to SO. 
%Similarly, we consider an implementable class of policies that take the form of a service compatibility structure, i.e., the policy induces a partition on the feature space of the individuals $\mathcal X$ to create distinct individual queues (wait lists), each of which will be eligible for a subset of resources. We define $\mathcal P : \mathcal X \rightarrow \mathcal Q$ as a function that assigns the individual $\bm x$ to one of the queues in the set $\mathcal Q$. Following the FCFS discipline, the policy assigns arriving resources to the individuals on the wait lists. Explicitly, we use $\pi(\bm X; M)$ to denote the policy corresponding to matching topology $M$. We note that in our setting $\mathcal P$ is not determined a priori (queues are not given). The only information available is the number of desired queues. We propose to find the function $\mathcal P$ as part of the policy optimization which we describe in more detail in Section~\ref{sec:solution}. 
%The definition  where $\mathcal Q:= \{1, \dots, Q\}$ is the set of queues, $\mathcal R:= \{1, \dots, T\}$ is the set of treatments/interventions (including ``no intervention''). Also, $\bm \lambda := \{\lambda_1, \dots, \lambda_Q\}, \bm \mu := \{\mu_1, \dots, \mu_Q\}$ denote the vector of arrival rates for the individual queues and resources, respectively.  
%\noindent\textbf{Policy Objectives. }Given a matching topology $M$, we use $\pi(\bm X; M)$ to denote the policy that allocates resources to individuals according to the FCFS principle. The policy is defined as the function $\pi_{M}(r; \bm x) = \mathbb{P}(R = r |\bm X_t = \bm x)$ as the probability that an individual arriving at time $t$ receives the resource $r$. We can evaluate the performance of a policy in terms of the expected of people exiting homelessness as $V(\pi_M) = \lim_{T \rightarrow \infty} \frac{1}{T} \mathbb{E}\left[\sum^{T}_{t = 1}\sum^{R}_{r = 1}\pi_M(r; \bm X, t)Y\left(r\right)\right]$, where the expectation is taken over all possible individual and resource arrival trajectories. Additionally, we wish to ensure the wait time of different queues is minimized and that the policy treats individuals from different groups fairly. We define wait time as $\mathbb{E}[]$
%Since individuals in the same queue have the same probability distribution of receiving the resources, we can equivalently define the policy as $\pi_{M}(r; \bm x) = \mathbb{P}(r |\mathcal P(\bm x))$. 
%We also study the system in the steady-state. In Section~\ref{sec:background},  Proposition~\ref{prop:steady-state} we provide the necessary and sufficient conditions for the system to arrive at the steady-state. Henceforth, we drop the dependence on time. 
%We note that in our setting $\mathcal P$ is not determined a priori (queues are not given). The only information available is the number of desired queues. We propose to find the function $\mathcal P$ as part of the policy optimization which we describe in more detail in Section~\ref{sec:solution}.
%$\pi_{M} : \mathcal X \rightarrow \Delta$ that maps individual's feature vector to a point in the unit simplex in $\mathbb R^{R}$. 
%According to the current recommended policy, upon entry to the system, each individual is assigned a NST score which determines their selection into different types of housing resources, i.e., the recommended policy is in the form of service compatibility graph that matches different score categories to specific resources. The actual assignment is then made according to a first-come-first-serve policy subject to the service compatibility restriction. In our setting, this can visualized as Figure~\ref{fig:HMIS-matching}.  According to this figure, individuals with score eight and above qualify for PSH, score 4 to 7 are assigned to the RRH wait list and finally individuals who score below 4 are not assigned to any of the housing interventions. 
%The existing policy $\bar{\pi}$ determines the eligibility of different individuals, i.e., $\bar{\pi}$ governs the allocation of housing resources to homeless individuals. The existing policy uses the NST score $s$ to prioritize individuals for the resources.
% \begin{equation}
%     \max_{\mathcal P , M \in \mathcal{M}} V(\pi_M).  
% \end{equation}
% In the above formulation, $\mathcal M$ encapsulate the set of fairness constraints and restrictions on the wait time. Next, we will define this set precisely. We study the system in the steady-state. In Section~\ref{sec:background},  Proposition~\ref{prop:steady-state} we provide the necessary and sufficient conditions for the system to arrive at the steady-state. Henceforth, we drop the variables' dependence on time. 
%The joint distribution of $\left(\bm X, \bm{Y}(t)\right)$ is unknown, however, we assume to have access to historical data in the form of the set $\mathcal D = \left\{(\bm x_i, t_i, y_i)\right\}^{N}_{i=1}$ where $\bm x^{i}$ is the realization of $\bm X$, the covariate vector collected for individual $i$. The dataset also contains the historical treatments of the individuals which can be either \textbf{R}apid-\textbf{R}e\textbf{H}ousing (RRH), \textbf{P}ermanent \textbf{S}upportive \textbf{H}ousing (PSH) or \textbf{S}ervice \textbf{O}nly (SO) (typically includes other services such as shelter etc.). Finally, $y^{i}(t_i) \in\{0,1\}$ is the observed outcome (we will drop the argument $t_i$ to simplify notation).
% \noindent\textbf{Fairness. }
% We also study group fairness, i.e., we assume individuals belong to different protected groups. We use random variable $G$ (collected as part of $\bm X$) to denote the group assignment. For example, $G$ can take values in $\{\text{Female, Male}\}$ or $\{\text{White}, \text{Black}, \text{Hispanics}\}$ if we consider fairness by gender or race, respectively. We note that in principle, our approach allows us to study intersectional fairness (fairness by multiple protected features). We will elaborate in the following sections. Additionally, we use $\bm Y$ to be the vector of the potential outcomes. We assume components of $\bm Y$ are binary. Finally, we let $T$ be the random variable for the treatment. Depending on the assigned treatment, we observe an outcome which we denote by $Y(T)$. 
\paragraph{Wait Time}%We now formalize the constraints required to achieve minimum wait time. 
%We use $\bm{W}(\vM)$ to denote the vector of average wait times of different queues. %The average wait time is given by the expression $\left(1/\lambda_{\mathcal Q}\right)\sum_{q \in \mathcal Q} \lambda_q W_q$.
Average wait time is dependent on the structure of the matching topology. For example, minimum average wait time is attainable in a fully FCFS policy where $\m_{\q\r} = 1\; \forall \q \in \sQ, \r \in \sR.$ In~\cite{Afeche2021OnSystem}, the authors characterize the general structural properties that impact average wait time. In particular, they show that under the heavy traffic condition, a matching system can be partitioned into a collection of complete resource pooling (CRP) subsystems that operate ``almost'' independently of
each other. A key property of this partitioning is that individuals that belong to the same CRP component experience the same average steady-state wait time. Furthermore, the average wait time is tied to the number of CRPs of a matching topology, where a single CRP achieves minimum average wait time. In~\cite{Afeche2021OnSystem},  the authors introduce necessary and sufficient constraints to ensure that the matching topology $\vM$ induces a single CRP component. {We adopt these constraints in order to achieve minimum wait time which we discuss next.}
%The constraints are explicitly defined in  Proposition~\ref{prop:crp}. 
%We build on the work in~\cite{Afeche2021OnSystem} to impose constraints on the matching topology $\vM$ that enforce minimum wait time. 
%For a formal definition of CRP, the reader is referred to~\cite{Stolyar2004MaxweightTraffic}. 
\iffalse
\begin{proposition}[\citet{Afeche2021OnSystem}, Proposition 8]
We define the non-negative decision variables $g^{(k)}_{qr} \geq 0 , (q, r, k) \in \sQ \times \sR \times \sQ$ as $Q$ sets of flow variables (indexed by the superscript $k \in \sQ$). The following set of constraints are necessary and sufficient to ensure that the matching topology $\vM = [\m_{\q\r}]$ induces a single CRP component.
\begin{subequations}
\begin{align*}
    & \sum_{\q \in \sQ} g_{\q\r}^{(k)} = \mu_\r & \forall \r \in \sR
    \\
    & \sum_{r \in \sR} g_{\q\r}^{(k)} = \lambda_{\q} - \frac{\delta}{|\sQ| - 1} & \forall \q \in \sQ\setminus\{k\}
    \\
    & \sum_{\r \in \sR} g_{\q\r}^{(k)} \leq Z \m_{\q\r} & \forall \q \in \sQ, \r \in \sR
    \\
    & \sum_{\r \in \sR} g_{\q\r}^{(k)} = \lambda_{k} + \delta, 
\end{align*}
\end{subequations}
where $\delta := \left(\prod_{\q \in \sQ}v_{\q}\prod_{\r \in \sR}v_{\r}\right)^{-1}$ and $\frac{w_{\q}}{v_{\q}} = \lambda_{\q}, \frac{w_{\r}}{v_{\r}} = \mu_{\r}$ are the rational number representations and $Z$ is defined as $Z := \max_{\q \in \sQ} \lambda_{\q} \max_{\r \in \sR} \mu_{\r} \left(1/\lambda_{\q} +  1/\mu_{\r} + (|\sQ|+|\sR|+1)^2 W \right)$, where $W := 1/2 \max \{\max_{\q\in\sQ} 1/\lambda_{\q},\max_{\r\in\sR} 1/\mu_{\r}\}$. 
\label{prop:crp}
\end{proposition}
\fi
\newar{Next, we present the final optimization formulation by incorporating both wait time and fairness considerations in Problem~\eqref{prob:policy-optimization}}.
\subsection{Optimization Formulation}\label{sec:optimization}
Suppose the joint distribution of $X$, $Y(\r) \; \forall \r \in \sR$ is known. Given a partitioning function $\P$ to assign individuals to queues,  problem~\eqref{prob:policy-optimization} can be solved via the MIO below. 
\begin{subequations}
    \begin{align}
    \max & \displaystyle \sum_{\q \in \sQ}\sum_{\r\in\sR} \tau_{\q\r}\f_{\q\r} 
    \\
    \text{s.t. } & \displaystyle \f_{\q\r},\nu_{\q\r} \in \mathbb R_{+}, \gamma_{r}, \theta_{q} \in \mathbb R & \forall \q \in \sQ, \r \in \sR
    \\
    & \displaystyle \m_{\q\r}, z_{\q\r} \in \{0,1\} &  \forall \q \in \sQ, \r \in \sR
    \\
    & \displaystyle g^{(k)}_{\q\r} \in \mathbb{R}_{+} & \forall \q, k \in \sQ, \r \in \sR
    \\
    & \displaystyle \sum_{q\in\sQ} \f_{\q\r} = \mu_{r} & \displaystyle \forall r \in \sR \label{eq-flow-1}
    \\
    & \displaystyle \sum_{\r\in\sR} \f_{\q\r} = \lambda_{q} & \displaystyle \forall q\in\sQ \label{eq-flow-2}
    \\
    & \displaystyle \f_{\q\r} \leq \lambda_{q}\mu_{\r}\left(\theta_{\q}+\gamma_{r}+\nu_{\q\r}\right) + Z(1-m_{qr}) & \forall q\in\sQ, r\in\sR \label{eq-kkt-1}
    \\
    & \displaystyle \f_{qr} \geq \lambda_{q}\mu_{r}\left(\theta_{q}+\gamma_{r}+\nu_{\q\r}\right)-Z(1 - m_{qr}) &  \forall q\in\sQ, r\in\sR \label{eq-kkt-2}
    \\
    & \displaystyle \f_{qr} \leq Z m_{qr} & \forall q\in\sQ, r\in\sR \label{eq-kkt-3}
    \\
    & \displaystyle \f_{qr} \leq Z z_{qr} &  \forall q\in\sQ, r\in\sR  \label{eq-kkt-4}
    \\
    & \displaystyle \nu_{\q\r} \leq (|\sQ|+|\sR|+1)W(1-z_{qr}) & \forall q\in\sQ, r\in\sR \label{eq-kkt-5}
    \\
    &  \displaystyle\sum_{\q \in \mathcal C} g_{qr}^{(k)} = \mu_r & \forall r \in \sR, k \in \sQ \label{eq-crp-1}
    \\
    &  \displaystyle\sum_{\r \in \sR} h_{qr}^{(k)} = \lambda_q - \frac{\delta}{|\sQ| - 1} & \forall q \in \sQ\setminus\{k\}, k \in \sQ  \label{eq-crp-2}
    \\
    &  \displaystyle\sum_{\r \in \sR} g_{qr}^{(k)} \leq Z m_{qr} & \forall q, k \in \sQ, r \in \sR \label{eq-crp-3}
    \\
    &  \displaystyle\sum_{r \in \sR}g_{qr}^{(k)} = \lambda_{k} + \delta  & \forall q, k \in \sQ \label{eq-crp-4}
    \\ 
    %&  \frac{1}{\lambda_{\sQ_g}}\sum_{q \in \sQ_g} \sum_{r \in \sR} f_{qr}\tau_{qr} + C \geq w & \forall g \in \mathcal G.
    & \vF \in \sF \label{eq-fairness}.
\end{align}
%\notepv{really hard to read all this.. big equations should not be in line + looks a little ugly since makes line spacing uneaven} 
In this formulation, $\delta := \left(\prod_{\q \in \sQ}v_{\q}\prod_{\r \in \sR}v_{\r}\right)^{-1}$ and $\frac{w_{\q}}{v_{\q}} = \lambda_{\q}, \frac{w_{\r}}{v_{\r}} = \mu_{\r}$ are rational number representations. $W := 1/2 \max \{\max_{\q\in\sQ} 1/\lambda_{\q},\max_{\r\in\sR} 1/\mu_{r}\}$, and $\textstyle Z := \max_{\q\in\sQ} \lambda_{q} \max_{\r \in \sR} \mu_{r} \left(\sum_{\q\in\sQ} 1/\lambda_{\q} +  \sum_{\r\in\sR} 1/\mu_{\r} + (|\sQ|+|\sR|+1)^2 W \right)$. 
\label{prob:MILP}
\end{subequations}
Constraints \eqref{eq-flow-1} and \eqref{eq-flow-2} are the flow balance constraints. Constants $W, Z$ ensure that constraints~\eqref{eq-kkt-1}-\eqref{eq-kkt-5} impose the KKT conditions of the quadratic program that approximates steady-state-flow for a matching topology $\vM$. Constraints~\eqref{eq-crp-1}-\eqref{eq-crp-4} enforce a single CRP component to ensure minimum wait time. 
Finally, constraint~\eqref{eq-fairness} collects the fairness constraints where we can use any of the aforementioned examples. In order to solve problem~\eqref{prob:MILP}, we need to estimate $\tau_{\q\r}$ and $\bm \lambda$ which depend of $\P$, as well as $\bm \mu$. 
\newar{Once the queues are fixed, estimating $\bm \lambda$ values are straightforward. In addition, $\bm \mu$ can be easily estimated from the historical provision of resources. In the next section, we discuss how to construct the queues and simultaneously estimate the $\tau_{\q\r}$ values.}

\section{Solution Approach}\label{sec:solution}

%In this work, we consider mappings in the form of axis-aligned tree structures (tree or forests) \notepv{why?} \notepv{it would be good to have an illustration of this idea; sounds really abstract right now}.
%In the previous section, we introduced the policy optimization assuming access to the joint distribution of the random variables $\bX$
%We note that the unknown parameters necessary in the set of waiting time constraints are the arrival rates which, once the matching model is constraints (e.g., the individuals queues), can be easily estimated from the observational data. On the contrary, building the queues, evaluating the policy value and the fairness constraints are faced with challenges as they are tied to the outcomes that are only partly observed. 
%In order to solve problem~\ref{prob:MILP}, we need to estimate $\tau_{\q\r}$ which {depends} on $\P$. \notepv{also need other parameters; i would move this part to the end of the previous section; otherwise not clear why we even need a solution approach (i.e this section)}
We first partition $\sX$ and then estimate CATE in each subset of the partition. We propose to use causal trees to achieve both tasks simultaneously~\cite{Wager2018EstimationForests}. Causal trees estimate CATE of binary interventions by partitioning the feature space into sub-populations that differ in the magnitude of their treatment effects. The method is based on regression trees, modified to estimate the goodness-of-fit of treatment effects. A key aspect of using causal trees for partitioning is that the cut points on features are such that the treatment effect variance within each leaf node is minimized. In other words, individuals who are similar in the treatment effect are grouped together in a leaf node. This results in queues that are tied to the treatment effect of resources which will result in improved policy value (see Section~\ref{sec:experiments}). 
% \begin{assumption}
% \begin{itemize}
% \item Stable Unit Treatment Value Assumption (SUTVA): It states the treatment that one unit (individual) receives does not change the potential outcomes of other units.
% \item Consistency: 
% %Formally, $Y=Y(\r)(\mathbb I(\R = \r)), \forall \r \in \sR$. 
% In words, $Y$ agrees with the potential outcome corresponding to the respective treatment. The implication of this assumption is that there are no two versions of a treatment such that $R=r$ under both versions but the
% potential outcome for $Y$ would be different under the alternative versions.
% \item Positivity: At each level of $\vX$, the probability of receiving any form of treatment is strictly positive. Mathematically,
% $$\mathbb{P}\left( \mathbb{P}(\R = \r |\vX = \vx) > 0 \right) = 1 \; \forall \r \in \sR \; \vx \in \sX.$$
% %where $\text{\rm{Supp}}(\bm X)$ is the support function of $\bm X$.
% \item Conditional Exchangeability: it states that individuals receiving a treatment should be considered exchangeable, with respect to potential outcomes $Y(\r), \r \in \sR$, with those not receiving it and vice versa. Mathematically, 
% $$
% \{Y(1), \dots, Y(|\sR|)\} \perp R |\vX = \vx. $$
% %where $\vY = \{Y(1), \dots, Y(|\sR|)\}$. 
% \end{itemize}
% \label{assum:causal-assum}
% \end{assumption}
\subsection{Assumptions}
Causal trees rely on several key assumptions which are standard in causal inference for treatment effect estimation~\cite{Hernan2013CausalBook}. These assumptions are {usually} discussed for the case of binary treatments. Below, we provide a generalized form of the assumptions for multiple treatments. 

\begin{assumption}[Stable Unit Treatment Value Assumption (SUTVA)]
The treatment that one unit (individual) receives does not change the potential outcomes of other units. 

\end{assumption}
%\newar{SUTVA can be viewed as a non-interferenceassumption. In the housing allocation }
\begin{assumption}[Consistency]
The observed outcome agrees with the potential outcome under the treatment received.
\end{assumption}
The implication of this assumption is that there are no different forms of each treatment which lead to different potential outcomes. In the housing allocation setting, this requires that there is only one version of PSH, RRH and SO.
\begin{assumption}[Positivity]
For all feature values, the probability of receiving any form of treatment is strictly positive{, i.e.,}
$$
\mathbb{P}(\R = \r |\vX = \vx) > 0 \; \forall \r \in \sR \; \vx \in \sX.$$
\end{assumption}
Th positivity assumption states that any individual should have a positive probability of receiving any treatment. Otherwise, there is no information about the distribution of outcome under some treatments and we will not be able to make inferences about it. In Section~\ref{sec:experiments}, we discuss the implications of this assumption in the context of HMIS data.
\begin{assumption}[Conditional Exchangeability]
Individuals receiving a treatment should be considered exchangeable, with respect to potential outcomes $Y(\r), \r \in \sR$, with those not receiving it and vice versa. Mathematically, 
$$
Y(1), \dots, Y(|\sR|) \perp R |\vX = \vx \; \forall \vx \in \sX.
$$
\end{assumption}
% \begin{assumption}[Conditional Exchangeability]
% Potential outcomes $\bm Y$ are independent of $R$ given $X$, i.e., $\bm Y \perp R |\bm X$. 
% \label{assum:exchange}
% \end{assumption}
% \begin{assumption}[Coverage]
% $
% \mathbb{P}\left( \mathbb{P}(R = r |\bm X = \bm x) > 0 \right) = 1 \; \forall \bm x \in \text{\rm{Supp}}(\bm X).
% $
% \label{assum:coverage}
% \end{assumption}
%These assumptions are standard in causal inference which allow the valid inference based on data. Assumption~\ref{assum:exchange} states that, given $\bm X$, the treatment assignment is random, hence, there is no dependence between $R$ and $\bm Y$ suggesting that we measured the right attributes to separate the effect of the outcome from the effect of intervention. Assumption~\ref{assum:coverage} states that the data generating distribution has a strictly positive probability of assigning any treatment to any individual. 

%In Section~\ref{sec:solution}, we discuss the validity of these assumptions in the context of housing allocation data collection. 
%Causal trees~\cite{Wang2017AAnalysis} have been previously used to identify heterogeneous treatment effect across health care providers and different groups of patients~\cite{Wang2017AAnalysis}. 
% \newar{The literature on off-policy evaluation offers several estimators to tackle this problem. We first make several assumptions. 
% \begin{assumption}[Conditional Exchangeability]
% Potential outcomes $\bm Y$ are independent of $R$ given $X$, i.e., $\bm Y \perp R |\bm X$. 
% \label{assum:exchange}
% \end{assumption}
% \begin{assumption}[Coverage]
% $
% \mathbb{P}\left( \mathbb{P}(R = r |\bm X = \bm x) > 0 \right) = 1 \; \forall \bm x \in \text{\rm{Supp}}(\bm X).
% $
% \label{assum:coverage}
% \end{assumption}
% These assumptions are standard in causal inference which allow the valid inference based on data. Assumption~\ref{assum:exchange} states that, given $\bm X$, the treatment assignment is random, hence, there is no dependence between $R$ and $\bm Y$ suggesting that we measured the right attributes to separate the effect of the outcome from the effect of intervention. Assumption~\ref{assum:coverage} states that the data generating distribution has a strictly positive probability of assigning any treatment to any individual. In Section~\ref{sec:solution}, we discuss the validity of these assumptions in the context of housing allocation data collection. }
%\notepv{need to define what this means (in the text)} 
Conditional exchangeability means that there are no unmeasured confounders that are a common cause of both treatment and outcomes. If unmeasured confounders exist, it is impossible to accurately estimate the causal effects. %In experimental settings, conditional exchangeability is obtained through stratified randomization. 
In observational settings, a decision-maker only relies on passive observations. As a result, in order to increase the plausibility of this assumption, researchers typically include as many features as possible in $\vX$ to ensure that as many confounders as possible between treatment and outcome are accounted for. In the housing allocation setting, the HMIS data contains a rich set of features (54 features) associated with different risk factors for homelessness which we use in order to estimate the treatment effects. In Section~\ref{sec:discussion}, we discuss the consequences of violating the above assumptions.

\subsection{Building the Partitioning Function}
Next, we describe our approach for estimating CATE. 
We first consider a simple case with binary treatments, i.e., $|\sR| = 2$ as causal trees work primarily for binary treatments.
After training the causal tree using the data on a pair of treatments, the leaves induce a partition on the feature space $\sX$. Hence, we can view the causal tree as the partitioning function $\P$ where each individual is uniquely mapped to a leaf node, i.e., a queue. 


\begin{wrapfigure}{r}{0.35\textwidth}
  \begin{center}
        \includegraphics[width=0.35\textwidth]{images/example.pdf}
  \end{center}
  \caption{Example partitioning by sample causal trees for PSH and RRH interventions.}
  \label{fig:example}
\end{wrapfigure}
Extending to the case of $|\sR| > 2$ is non-trivial. 
Assuming $\r = 1$ is the baseline intervention, we  construct $|\sR|-1$ separate causal trees to estimate CATE for $\r \in \sR\setminus\{1\}$. We denote the resulting causal trees or partitioning functions $\P_{\r}:\sX \rightarrow \sQ \; \forall \r \in \sR\setminus\{1\}$. We define $\sX_{\r}(\q) = \left\{ \vx \in \sX: \P_{\r}(\vx) = \q \right\} \forall \r \in \sR\setminus\{1\}, \q \in \sQ$ as the set of all individuals who belong to queue $\q$ according to partitioning function $\P_r$. Also, let $\q_{\r} = \P_{\r}(\vx)$.
In order to aggregate the individual partitioning functions to obtain a unified partition on $\sX$, we consider the intersections of $\sX_{\r}(\q)$ created by each tree. We define subsets $\sX(\q_{1}, \dots, \q_{|\sR|-1}) = \bigcap^{|\sR|-1}_{\r = 1} \sX_{\r}(\q_{\r})$ for all combinations of $\q_\r \in \sQ$. We can view $\sX(\q_{1}, \dots, \q_{|\sR|-1})$ as a new (finer) partition on $\sX$.
%Using the intersections of subsets $\sX_{\r}(\q)$, we construct a new (finer) partition on $\sX$.
%We now describe how to aggregate the individual partitioning functions $\P_{\r}, \r \in \sR$ to obtain a unified partition using the intersection of these $\sX_{\r}$.
%Suppose $\vx \in \sX_{\r}(\q_\r) \; \forall \r \in\sR\setminus\{1\}$, where $\q_\r = \P_{r}(\vx)$. It holds that $\vx \in \bigcap^{|\sR|-1}_{\r = 1}\sX_{\r}(\q_{\r})$. 
%That is, an individual who belongs to queues $\q_{\r}$ (in each tree $\r$), also belongs to the set $\sX_{q_1,\dots,q_{|\sR|-1}} = \left\{\vx : \P_{\r}(\vx) = \q_{1} \land \dots \land  \P_{|\sR|-1}(\vx) = \q_{|\sR|-1} \right\}$. The subsets $\sX_{1,\dots,|\sR|-1}$ can be viewed as a new (finer) partition on $\sX$. 
%Suppose $\vx \in \sX_{2}(\q)$ and $\vx \in \sX_{3}(\q')$, where $q = \P_{2}(\vx)$ and $\q' = \P_{3}(\vx)$. It holds that $\vx \in \sX_{2}(\q) \cap \sX_{3}(\q')$. That is, an individual who belongs to queues $\q$ and $\q'$ (based on two different partitioning functions), also belongs to the set $\sX_{\q, \q'} = \left\{\vx : \P_{2}(\vx) = \q \land \P_{3}(\vx) = \q' \right\}$. The subsets $\sX_{\q, \q'} \; \forall \q, \q' \in \sQ$ can be viewed as a new (finer) partition on $\sX$. 
We illustrate with an example using the housing allocation setting. Suppose we have constructed two causal trees for PSH and RRH according to Figure~\ref{fig:example} such that PSH tree splits the vulnerability score into intervals of $[0,6], [7, 10], [11, 17]$ and RRH creates $[0, 8], [9, 17]$ subsets. According to our procedure, the final queues are constructed using the intersection of these subsets. In other words, we obtain $[0, 6], [7, 8], [9, 10], [11, 17]$ which corresponds to four queues. \newar{Building queues as the intersection of the tree subsets may result in a large number of queues. However, even though the size of the optimization problem is quadratic in the number of queues, in practice the problem solves relatively quickly (in seconds) for queue number up to 30 which is far more than what is typically seen in practice. In addition, the granularity of the partition, and subsequently the number of queues, can be controlled through the tree depth or the minimum allowable number of data points in each leaf, both of which are adjustable parameters in causal trees. It is noteworthy that while fewer queues result in models that are easily interpretable, more queues allow the decision-makers to leverage the heterogeneity in treatment effect to target the resources to the right individuals, hence achieving higher-valued policies. We explore this trade-off in the experimental result section.}

%\newar{In practice, fewer queues offer more simplicity and result in models that are easily interpretable, however, more queues allow the decision-makers to leverage the heterogeneity in treatment effect to target the resources to the right individuals, hence achieving higher-valued policies. We investigate this trade-offs in the experimental results section. } .  Further, even though the size of the optimization problem is quadratic in the number of queues, in practice the problem solves relatively quickly


Finally, in order to estimate $\tau_{\q\r}$, we should avoid using the estimates from each individual tree.  
%The benefit of constructing the queues in this fashion is that the causal tree aims to minimize the treatment effect variation within each leaf node. 
%As a result, data points (individuals) that fall under the same leaf node will exhibit similar response to the treatment they are assigned to which is desirable when constructing the queues. 
%each causal trees After we constructed the queues, it is important to re-evaluate the treatment effects for each queue. 
The reason is that each tree estimates $\mathbb{E}[Y(\r) - Y(1) |\P(\vX) = \q, \R \in \{1, \r\}] \; \forall \r \in \sR\setminus\{1\}$. That is, a subset of the data associated with a pair of treatments is used to build each tree. Therefore, $\tau_{\q\r}$ values are not generalizable to the entire population and need to be re-evaluated over all data points that belong to a subset. 
We adopt Doubly Robust estimator (DR) for this task. Proposed in~\cite{Dudik2011DoublyLearning}, DR combines an outcome regression with a model for the treatment assignment (propensity score) to estimate treatment effects. DR is an unbiased estimate of treatment effects, if at least one of the two models are correctly specified. Hence, it has a higher chance of reliable inference. CATE estimates $\hat{\tau}_{\q\r}$ are provided below.
\begin{equation*}
    \hat{\tau}_{\q\r} = \frac{1}{|\mathcal I_{\q}|}\sum_{i\in \mathcal I_{\q}}\left(\hat{y}(\bm X_i, r) + \left(Y_i - \hat{y}(\bm X_i, R_i)\right)\frac{\mathbb{I}(\R_i = r)}{\bar{\pi}(\R_{i}|\vX_i)}\right) - \frac{1}{|\mathcal I_{\q}|}\sum_{i\in \mathcal I_{\q}}\left(\hat{y}(\bm X_i, 1) + \left(Y_i - \hat{y}(\bm X_i, R_i)\right)\frac{\mathbb{I}(\R_i = 1)}{\bar{\pi}(\R_{i}|\vX_i)}\right) , 
\end{equation*}
where $\mathcal I_{\q} := \{i \in \{1,\dots,N\}: \P(\vX_{i}) = \q\}$ is the set of indices in the historical data that belongs to $\q$. Further, $\hat{y}$ and $\bar{\pi}$ are the outcome and historical policy (i.e., propensity score) models, respectively. 


We end this section by discussing a practical consideration which is a desire to design policies that depend on low-dimensional features, such as risk scores. In cases that we only use risk scores, not the full feature vector, it is critical that they satisfy the causal assumptions. We provide a risk score formulation that satisfies this requirement.
%\notepv{i don't think this is true: provided you are allowed to use all covariates to estimate both mu and the outcome in direct method; the policy can depend on a lower dimensional feature vector}
\begin{proposition}
We define risk score functions as $S_r(\vx) = \mathbb{P}[Y(\r) = 1 |\vX = \vx] \; \forall \r \in \sR$. Suppose $\bm S \in \mathcal S$ is a (random) vector
%$\bm S = (S_1, \dots, S_R), \bm S \in \mathcal S$ 
of risk scores. Also, let $\bm Y = (Y(1),\dots,Y(|\sR|))$ be the vector of potential outcomes. The following statements hold:
\begin{enumerate}
    \item If $\bm Y \perp \R |\vX$, then $\bm Y \perp \R |\bm S$. 
    \item If $\mathbb{P}\left( \mathbb{P}(\R = \r |\vX = \vx) > 0 \right) = 1 \; \forall \vx \in \sX$, then $\mathbb{P}\left( \mathbb{P}(\R = \r |\bm S = \bm s) > 0 \right) = 1 \; \forall \bm s \in \mathcal S.$
\end{enumerate}
\label{prop:feature-summarization}
\end{proposition}
Under causal assumptions, $S_r(\vx) = \mathbb{P}(Y(\r) = 1 |\vX = \vx, \R = \r) = \mathbb{P}(Y = 1 |\vX = \vx, \R = \r)$, which relies on observed data, rather than counterfactuals. According to Proposition~\ref{prop:feature-summarization}, as in general individuals respond differently to various treatments, one risk score per resource may be required in order to summarize the information of $\vX$. \newar{Alternatively, one can utilize the entire set of features in the causal tree and to learn the propensity and outcome models used in the treatment effect estimators.}
%In our numerical results, we use the entire feature vector to learn the propensity and outcome models which we use in to construct the causal tree.
%So far, we have assumed access to a feature vector $\vX$ that satisfies the causal assumptions. In practice it is often desirable to design policies that depend on lower-dimensional features, such as a risk score. To do so, we need to ensure that the aforementioned assumptions still hold once we replace $\vX$ with a risk score. In the general case, one risk score per resource is required. The reason is that risk factors under different resources may be different and an individual who responds well to treatment one, may not necessarily respond well to another treatment. 
% \begin{proof}
% We first prove part one and we show the conditional independence for each component $Y_r$ of the potential outcome vector.  The proof is in the same vein as the balancing scores in the causal inference literature which as essentially a low-dimensional summary of the relevant covariate space, can facilitate causal inference for observational data in settings with many covariates.
% \begin{align*}
%     \mathbb{P}(Y_{r} = 1|\bm S, R) & =  \mathbb{E}[Y_{r} |\bm S, R] \\
%     & = \mathbb{E}\left[\mathbb{E}\left[Y_{r} |\bm S, R, \bm X \right]\,\vert\,\bm S, R\right] \\
%     & = \mathbb{E}\left[\mathbb{E}\left[Y_{r} |\bm S, \bm X \right]\,\vert\,\bm S, R\right] \\
%     & = \mathbb{E}\left[\mathbb{E}\left[Y_{r} |\bm X \right]\,\vert\,\bm S, R\right] \\
%     & = \mathbb{E}\left[S_r\,\vert\,\bm S, R\right] \\
%     & = S_r, 
% \end{align*}
% where the third line follows the assumption of the proposition and the fourth line holds since $\bm S$ is essentially a function of $\bm X$ and can be dropped. 
% We also show
% \begin{align*}
%     \mathbb{P}(Y_{r} = 1|\bm{S}) & =  \mathbb{E}[Y_{r} |\bm S] \\
%     & = \mathbb{E}\left[\mathbb{E}\left[Y_{r} |\bm S, \bm X \right]\,\vert\,\bm S\right] \\
%     & = \mathbb{E}\left[\mathbb{E}\left[Y_{r} | \bm X \right]\,\vert\,\bm S\right] \\
%     & = \mathbb{E}\left[S_r\,\vert\,\bm S\right] \\
%     & = S_r.
% \end{align*}
% We proved $\mathbb{P}(Y_{r} = 1|\bm S, T) = \mathbb{P}(Y_{r} = 1|\bm S)$. 
% We now prove the second part of the proposition. 
% \begin{align*}
%     \mathbb{P}\left( \mathbb{P}(R = r |\bm X = \bm x) > 0 \right) = 1 & \Rightarrow \mathbb{P}\left( \mathbb{P}(R = r, \bm X = \bm x) > 0 \right) = 1\\
% \end{align*}
% \begin{align*}
%     \mathbb{P}\left( \mathbb{P}(R = r, \bm X = \bm x) > 0 \right) & =  \mathbb{P}\left( \mathbb{P}(R = r, \bm X = \bm x, \bm S = \bm s) > 0 \right) \\
%     & \leq \mathbb{P}\left( \mathbb{P}(R = r, \bm S = \bm s) > 0 \right). 
% \end{align*}
% It follows that $\mathbb{P}\left( \mathbb{P}(R = r, \bm S = \bm s) > 0 \right) = 1$ for all values of $\bm s$. 
% \end{proof}

%Next, we create the queues by considering the intersection of all the partitioning functions. Mathematically, we define $\mathcal Q^{r}, \; r \in \{2, \dots, R\}$ to denote the set of leaves associated with the causal trees, each estimating CATE for resource $r $ compared to $r = 1$ (the baseline resource). Each individual in the dataset belongs uniquely to one of the $(q_{2}, \dots, q^{r})$ vectors, where $ q^{r} \in \mathcal{Q}^{r}, \forall r \in \{2, \dots, R\}$. Since there are at most $\bigcup^{|\mathcal{Q}^2 \times \mathcal{Q}_r|}_{q=1} \mathcal {Q}^{r}$. 

%We use $\mathcal {X}_q, \; q \in \mathcal Q_1 \times \mathcal Q_2$ to indicate each subset. Note that $\mathcal X = \bigcup^{|\mathcal{Q}_1 \times \mathcal{Q}_2|}_{q=1} \mathcal {X}_q$. The overall treatment effect with respect to each of the treatments are defined as

% \subsection{Policy Optimization}
% We now present a mixed integer linear program (MILP) to solve the optimization Problem~\eqref{prob:policy-optimization}. 
% \begin{subequations}
%     \begin{align}
%     \max & \displaystyle \sum_{
%     q\in\mathcal Q,
%     r\in\mathcal R} \tau_{qr}f_{qr} 
%     \\
%     \text{s.t. } & \displaystyle f_{qr},\nu_{qr} \in \mathbb R_{+}, \gamma_{qr}, \theta_{q} \in \mathbb R & \forall q\in\mathcal Q, t\in\mathcal R
%     \\
%     & \displaystyle m_{qr}, z_{qr} \in \{0,1\} &  \forall q\in\mathcal Q, r \in \mathcal R
%     \\
%     & \displaystyle \sum_{q\in\mathcal Q} f_{qr} = \mu_{r} & \displaystyle \forall r \in \mathcal R.
%     \\
%     & \displaystyle \sum_{t\in\mathcal R} f_{qr} = \lambda_{q} & \displaystyle \forall q\in\mathcal Q.
%     \\
%     & \displaystyle f_{qr} \leq \lambda_{q}\mu_{r}\left(\theta_{q+\gamma_{r}+\nu_{qr}}\right) + Z(1-m_{qr}) & \forall q\in\mathcal Q, r\in\mathcal R
%     \\
%     & \displaystyle f_{qr} \geq \lambda_{q}\mu_{r}\left(\theta_{q+\gamma_{r}+\nu_{qr}}\right)-Z(1 - m_{qr}) &  \forall q\in\mathcal Q, r\in\mathcal R
%     \\
%     & \displaystyle f_{qr} \leq Z m_{qr} & \forall q\in\mathcal Q, r\in\mathcal R
%     \\
%     & \displaystyle f_{qr} \leq Z z_{qr} &  \forall q\in\mathcal Q, r\in\mathcal R 
%     \\
%     & \displaystyle \nu_{qr} \leq (|\mathcal Q|+|\mathcal R|+1)W(1-z_{qr}) & \forall q\in\mathcal Q, r\in\mathcal R 
%     \\
%     &  \displaystyle\sum_{q \in \mathcal C} g_{qr}^{(k)} = \mu_r & \forall r \in \mathcal R
%     \\
%     &  \displaystyle\sum_{r \in \mathcal R} h_{qr}^{(k)} = \lambda_q - \frac{\delta}{n - 1} & \forall q \in \mathcal Q\setminus\{k\}
%     \\
%     &  \displaystyle\sum_{r \in \mathcal R} g_{qr}^{(k)} \leq Z m_{qr} & \forall q \in \mathcal Q, r \in \mathcal R
%     \\
%     &  \displaystyle\sum_{r \in \mathcal R}g_{qr}^{(k)} = \lambda_{k} + \delta 
%     \\ 
%     &  \frac{1}{\lambda_{\mathcal Q_g}}\sum_{q \in \mathcal Q_g} \sum_{r \in \mathcal R} f_{qr}\tau_{qr} + C \geq w & \forall g \in \mathcal G.
% \end{align}
% \label{prob:MILP}
% where $\displaystyle W := 1/2 \max \{\max_{q\in\mathcal Q} 1/\lambda_{q},\max_{r\in\mathcal R} 1/\mu_{r}\}$, and $ \displaystyle Z := \max_{q\in\mathcal Q} \lambda_{q} \max_{t\in\mathcal R} \mu_{r} \left(1/\lambda_{q} +  1/\mu_{r} + (|\mathcal Q|+|\mathcal R|+1)^2 W \right)$. 
% \end{subequations}
% In this formulation, constraints (3d) and (3e) are the flow balance constraints. The constants $W, Z$ ensure that the constraints (3f)-(3j) impose the KKT conditions of the quadratic program that approximates the steady-state-flow for any matching topology $M$. Constraints (3k)-(3n) enforce a single CRP component to ensure minimum wait time. See~\cite{Afeche2021OnSystem} for more details. Finally, constraints (3o) are the fairness constraints, where $w$ is an input parameter. In the experiments we set $w$ to the maximum value for which the above optimization problem is feasible. 



